Fast Homotopy for Spacecraft Rendezvous Trajectory Optimization with Discrete Logic

This paper presents a computationally efficient optimization algorithm for solving nonconvex optimal control problems that involve discrete logic constraints. Traditional solution methods for these constraints require binary variables and mixed-integer programming, which is prohibitively slow and computationally expensive. This paper targets a fast solution that is capable of real-time implementation onboard spacecraft. To do so, a novel algorithm is developed that blends sequential convex programming and numerical continuation into a single iterative solution process. Inside the algorithm, discrete logic constraints are approximated by smooth functions, and a homotopy parameter governs the accuracy of this approximation. As the algorithm converges, the homotopy parameter is updated such that the smooth approximations enforce the exact discrete logic. The effectiveness of this approach is numerically demonstrated for a realistic rendezvous scenario inspired by the Apollo Transposition and Docking maneuver. In under 15 seconds of cumulative solver time, the algorithm is able to reliably find difficult fuel-optimal trajectories that obey the following discrete logic constraints: thruster minimum impulse-bit, range-triggered approach cone, and range-triggered plume impingement. The optimized trajectory uses significantly less fuel than reported NASA design targets.

==> latex_common/PykZ/pykz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% PykZ
%
% A package that combines the speed of Python for numerical calculation and the
% drawing capabilities of TikZ, to make publication-quality drawing faster.
%
% Some conventions:
%
%   \@pik@<name> : PykZ internal key <name>
%   \@piv@<name> : PykZ internal variable <name>
%   \@pic@<name> : PykZ internal command <name>
%   @pie@<name> : PykZ internal environment <name>
%
% Danylo Malyuta, 2020
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Load packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{filecontents}
\usepackage{fancyvrb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\gdef\@piv@python@delay{0.5} % Startup wait for Python server

\newcommand{\pykzinit}[1]{
  % ---------------------------------------------------------
  %
  % Initialization of PykZ.
  % Starts the Python background server process.
  % Must be called before doing anything that uses PykZ.
  %
  % ---------------------------------------------------------
  \xdef\@piv@relpath{#1}
  % Start a background Python server
\begin{@pie@shell}
curdir=$(pwd) $() &&
cd \@piv@relpath &&
python server.py &
\end{@pie@shell}
  % Allow some start-up time for Python
\begin{@pie@shell}
sleep \@piv@python@delay
\end{@pie@shell}
  % Determine path to directory where latex_common resides
  \pykzmathinline[@piv@pypath]{'\@piv@relpath'[:'\@piv@relpath'.find('latex_common')]}
  % Include mathematical plotting functionality
  \input{\@piv@relpath/pyplot.tex}
}

\NewEnviron{@pie@shell}{%
  \immediate\write18{\BODY}%
}

\newenvironment{pykzpicture}[1][]{%
  % ---------------------------------------------------------
  %
  % A wrapper of the tikzpicture environment, which does all the PykZ
  % initialization in the background
  %
  % Parameters
  % ----------
  % #1 : same options as you would pass tikzpicture
  % #2 : relative location of PykZ directory
  %
  % ---------------------------------------------------------
  %
  % -------------------------------------
  % Check if 3D required
  % -------------------------------------
  \edef\@threed{3d}%
  \pykzmathinline[@use@threed]{'\@threed' in str('#1')}%
  \pykzmathinline[@tikz@opts]{str('#1').replace('\@threed,','').
    replace(',\@threed','').replace('\@threed','')}%
  % -------------------------------------
  % Start the tikzpicture
  % -------------------------------------
  \tikzset{%
    apply style/.code={%
      \tikzset{#1}%
    }%
  }%
  \begin{tikzpicture}[
    % Rounded line ends
    line cap=round,
    % Bevelled (non-sharp) polygon corners
    line join=bevel,
    % User commands
    apply style/.expand once=\@tikz@opts]
    %
    % -------------------------------------
    % Common styles
    % -------------------------------------
    \tikzset
    {
      % No default separation
      every node/.append style=
      {
        inner sep=0,
        outer sep=0
      },
      % Default arrow
      arrow/.append style=
      {
        -latex
      },
      % Text labels
      label/.append style=
      {
        outer sep=1
      },
      % Bezier curve controls style
      bezier/.style={
        postaction={
          decoration={
            show path construction,
            curveto code={
              \draw [blue]
              (\tikzinputsegmentfirst) -- (\tikzinputsegmentsupporta)
              (\tikzinputsegmentlast) -- (\tikzinputsegmentsupportb);
              \fill [red, opacity=0.5]
              (\tikzinputsegmentsupporta) circle [radius=.5ex]
              (\tikzinputsegmentsupportb) circle [radius=.5ex];
            }
          },
          decorate
        }}
    }%
    %
    % -------------------------------------
    % Activate 3D plot
    % -------------------------------------
    \ifthenelse{\equal{\@use@threed}{True}}{
      \xdef\@piv@td@main@alt{60}%
      \xdef\@piv@td@main@azi{125}%
      \tdplotsetmaincoords{\@piv@td@main@alt}{\@piv@td@main@azi}%
      \pykzmathinline[@piv@td@R]{(np.eye(3)).tolist()}%
    }{}
    \pykzmathinline[@threed@cmd]{'tdplot_main_coords' if (\@use@threed) else ''}%
    \begin{scope}[\@threed@cmd]%
      %
      % -------------------------------------
      % User code
      % -------------------------------------
    }
    % BODY
    {
    \end{scope}%
  \end{tikzpicture}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Math library
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\pykzexec}[1]{%
  % ---------------------------------------------------------
  %
  % Call a function in pykz_custom.py, and store result in
  % local variables of Python session.
  %
  % ---------------------------------------------------------
\begin{@pie@shell}
cd \@piv@relpath && ./client "<exec> #1"
\end{@pie@shell}%
}

\newcommand{\pykzmathinline}[2][]{%
  % ---------------------------------------------------------
  %
  % Send one-line math command to Python, and store result in \out.
  %
  % ---------------------------------------------------------
\begin{@pie@shell}%
curdir=$(pwd) $() &&
cd \@piv@relpath &&
./client "#2" &&
mv result.tex $curdir $()
\end{@pie@shell}%
  \input{result.tex}%
  \ifthenelse{\equal{\out}{PYKZ_FAIL}}{%
    \PackageError{PykZ}{Python failed to process your command}{%
      Is your command proper Python syntax?}%
  }{}%
  \ifthenelse{\equal{#1}{}}{}{\expandafter\xdef\csname #1\endcsname{\out}}%
}

\newenvironment{pykzmathblock}
% ---------------------------------------------------------
%
% Save a block of Python code in a file accessible to PykZ
% for later execution.
%
% ---------------------------------------------------------
{\VerbatimOut{pykz_custom.py}}
{\endVerbatimOut
\begin{@pie@shell}
mv pykz_custom.py \@piv@pypath
\end{@pie@shell}
}

\newcommand{\pykzmathfunction}[1]{
  % ---------------------------------------------------------
  %
  % Call a function in pykz_custom.py, and store result in
  % local variables of Python session.
  %
  % ---------------------------------------------------------
\begin{@pie@shell}
cd \@piv@relpath && ./client "<function> #1"
\end{@pie@shell}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Drawing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\shift}[2]{%
  %
  % Shift a point #1 by amount #2.
  %
  ($(#1)+(#2)$)%
}

\renewcommand{\bezier}[2]{%
  % ---------------------------------------------------------
  %
  % Bezier curve controls.
  %
  % Parameters
  % ----------
  % #1 : angle:radius for start point control
  % #2 : angle:radius for end point control
  %
  % ---------------------------------------------------------
  .. controls ++(#1) and ++(#2) ..}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Beamer tools
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{pageplace}[1]
{
  \xdef\@pos@args{#1}
  \pykzpicture[remember picture,
  overlay,
  shift={(current page.center)}]
  \pykzmathinline[@arg@length]{len([\@pos@args])}
  \ifthenelse{\equal{\@arg@length}{2}}{
    % Direct position
    \pykzmathinline[@pos@x]{str([\@pos@args][0]).replace(chr(39),'')}
    \pykzmathinline[@pos@y]{str([\@pos@args][1]).replace(chr(39),'')}
    \dimensionalize{\@pos@x,\@pos@y}
  }{
    % Position using grid
    \tikzmath{
      \@page@width = \paperwidth;
      \@page@height = \paperheight;
    }
    \pykzmathinline[@pos@x]{(([\@pos@args][3]-0.5)/[\@pos@args][1]-0.5)*\@page@width}
    \pykzmathinline[@pos@y]{(-([\@pos@args][2]-0.5)/[\@pos@args][0]+0.5)*\@page@height}
    \dimensionalize{\@pos@x,\@pos@y}
  }
  \coordinate (loc) at (\@pos@x,\@pos@y);
}{
  \endpykzpicture
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Utilities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\convertto#1#2{\strip@pt\dimexpr #2*65536/\number\dimexpr 1#1}
\define@key{@pik@keys}{unit}{\def\@@@unit{#1}}
\newcommand{\dimensionalize}[2][]{%
  %
  % Append to #1 the unit \@@@unit.
  % Common use case is to append "pt" to a tikzmath output.
  %
  % -- Parameters
  \setkeys{@pik@keys}{unit=pt,#1}%
  % -- Function body
  \foreach \@@var in {#2} {%
    \ifthenelse{\equal{\@@@unit}{}}{%
      \pykzmathinline{'\@@var'[:-2]}%
      \expandafter\xdef\@@var{\out}%
    }{%
      \tikzmath{\@@@@value=\@@var;}% % to pt
      \def\@pt@unit{pt}%
      \xdef\@@@@tmp{\@@@@value\@pt@unit}% % append "pt" unit
      \expandafter\xdef\@@var{\convertto{\@@@unit}{\@@@@tmp}\@@@unit}% % convert to target unit
    }%
  }%
}

\define@key{@pik@keys}{amount}{\def\@@amount{#1}}
\newcommand{\counter@increment}[2][]{%
  %
  % Increments counter #2 by increment amount #1 (default: 1).
  %
  % -- Parameters
  \setkeys{@pik@keys}{amount=1,#1}%
  % -- Function body
  \tikzmath{\@@counter@next=int(#2+\@@amount);}%
  \xdef#2{\@@counter@next}%
}

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/PykZ/pyplot.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Plotting with PykZ
%
% A package that provides facilities for making plots of mathematical functions
% using PykZ.
%
% Some conventions:
%
%   \@pyplot@<name> : PykZ plotting variable
%   \pyplot@<name> : PykZ plotting function
%   \pyplot@internal@<name> : PykZ plotting internal function, don't touch!
%
% Danylo Malyuta, 2021
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Working with layers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@pykz@layers{main}

% Add a new layer behind all current layers
\newcommand{\pykz@add@layer@below}[1]{
  \pgfdeclarelayer{#1}
  \xdef\@pykz@layers{#1,\@pykz@layers}
  \pgfsetlayers{\@pykz@layers}
}

% Add a new layer in front of all current layers
\newcommand{\pykz@add@layer@above}[1]{
  \pgfdeclarelayer{#1}
  \xdef\@pykz@layers{\@pykz@layers,#1}
  \pgfsetlayers{\@pykz@layers}
}

% Define a layer "in front"
\pykz@add@layer@above{pyplot fg}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plotting variables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\@pyplot@arrow{Stealth[round]}
\def\@pyplot@unit{cm}
\def\@pyplot@clip{True}
\def\@pyplot@plotarea@x@size{2}
\def\@pyplot@plotarea@y@size{2}
\def\@pyplot@plotarea@xmin{-1}
\def\@pyplot@plotarea@xcenter{0}
\def\@pyplot@plotarea@xmax{1}
\def\@pyplot@plotarea@ymin{-1}
\def\@pyplot@plotarea@ycenter{0}
\def\@pyplot@plotarea@ymax{1}
\def\@pyplot@axarea@pad@left{0}
\def\@pyplot@axarea@pad@right{0}
\def\@pyplot@axarea@pad@top{0}
\def\@pyplot@axarea@pad@bottom{0}
\def\@pyplot@map@precision{4}
\def\@pyplot@python@maxchar{1015}
\def\@pyplot@background@color{white}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Drawing styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzset{
  pyplot axis/.style={
    -\@pyplot@arrow,
    black
  },
  pyplot axis label/.style={},
  pyplot plot area debug/.style={
    dashed,
    opacity=0.5
  },
  pyplot mark position/.style args={#1(#2)}{
    postaction={
      decorate,
      decoration={
        markings,
        mark=at position #1 with \coordinate (#2);
      }
    }
  },
  pyplot major tick/.style={
    line width=0.3
  },
  pyplot major tick label/.style={
    inner sep=0.03\@pyplot@unit
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Public functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Define the units. In all commands, leave numbers dimensionles!
\newcommand{\pyplot@set@unit}[1]{
  \xdef\@pyplot@unit{#1}
}

% Define the background color
\newcommand{\pyplot@set@bg}[1]{
  \xdef\@pyplot@background@color{#1}
}

% Set whether the plotted function coordinates are clipped before being
% returned to the user
\newcommand{\pyplot@set@clip}[1]{
  \xdef\@pyplot@clip{#1}
}

% Define the plot size
\newcommand{\pyplot@set@size}[2]{
  \xdef\@pyplot@plotarea@x@size{#1*1\@pyplot@unit}
  \xdef\@pyplot@plotarea@y@size{#2*1\@pyplot@unit}
}

% Define the x-axis limits
\define@key{@pyplot@keys}{center}{\def\@pyplot@plotarea@center{#1}}
\newcommand{\pyplot@set@xlim}[3][]{
  \setkeys{@pyplot@keys}{center=\@pyplot@plotarea@xcenter,#1}%
  \xdef\@pyplot@plotarea@xcenter{\@pyplot@plotarea@center}
  \xdef\@pyplot@plotarea@xmin{#2}
  \xdef\@pyplot@plotarea@xmax{#3}
}

% Define the y-axis limits
\newcommand{\pyplot@set@ylim}[3][]{
  \setkeys{@pyplot@keys}{center=\@pyplot@plotarea@ycenter,#1}%
  \xdef\@pyplot@plotarea@ycenter{\@pyplot@plotarea@center}
  \xdef\@pyplot@plotarea@ymin{#2}
  \xdef\@pyplot@plotarea@ymax{#3}
}

% Define the padding around the plot area
\define@key{@pyplot@keys}{left}{\def\@pyplot@axarea@pad@left@key{#1}}
\define@key{@pyplot@keys}{right}{\def\@pyplot@axarea@pad@right@key{#1}}
\define@key{@pyplot@keys}{top}{\def\@pyplot@axarea@pad@top@key{#1}}
\define@key{@pyplot@keys}{bottom}{\def\@pyplot@axarea@pad@bottom@key{#1}}
\newcommand{\pyplot@set@padding}[1]{
  \setkeys{@pyplot@keys}{left=\@pyplot@axarea@pad@left,#1}%
  \setkeys{@pyplot@keys}{right=\@pyplot@axarea@pad@right,#1}%
  \setkeys{@pyplot@keys}{top=\@pyplot@axarea@pad@top,#1}%
  \setkeys{@pyplot@keys}{bottom=\@pyplot@axarea@pad@bottom,#1}
  \xdef\@pyplot@axarea@pad@left{\@pyplot@axarea@pad@left@key*1\@pyplot@unit}
  \xdef\@pyplot@axarea@pad@right{\@pyplot@axarea@pad@right@key*1\@pyplot@unit}
  \xdef\@pyplot@axarea@pad@top{\@pyplot@axarea@pad@top@key*1\@pyplot@unit}
  \xdef\@pyplot@axarea@pad@bottom{\@pyplot@axarea@pad@bottom@key*1\@pyplot@unit}
}

% Draw the axes
\define@key{@pyplot@keys}{showarea}{\def\@pyplot@show@area@debug{#1}}
\define@key{@pyplot@keys}{yaxloc}{\def\@pyplot@y@axis@draw@location{#1}}
\define@key{@pyplot@keys}{xaxloc}{\def\@pyplot@x@axis@draw@location{#1}}
\newcommand{\pyplot@draw@axes}[1][]{
  \setkeys{@pyplot@keys}{showarea=false,#1}
  \setkeys{@pyplot@keys}{yaxloc=center,#1}
  \setkeys{@pyplot@keys}{xaxloc=center,#1}

  \coordinate (pyplot origin) at (0,0);

  % Adjust size for padding
  \tikzmath{
    \@pyplot@plotarea@x@size@padded = \@pyplot@plotarea@x@size-
    \@pyplot@axarea@pad@left-\@pyplot@axarea@pad@right;
    \@pyplot@plotarea@y@size@padded = \@pyplot@plotarea@y@size-
    \@pyplot@axarea@pad@top-\@pyplot@axarea@pad@bottom;
  }
  \dimensionalize{\@pyplot@plotarea@x@size@padded, \@pyplot@plotarea@y@size@padded}

  % ..:: x-axis ::..

  \pgfmathsetmacro{\@pyplot@negative@frac}{%
    (\@pyplot@plotarea@xcenter-\@pyplot@plotarea@xmin)/
    (\@pyplot@plotarea@xmax-\@pyplot@plotarea@xmin)}
  \pgfmathsetmacro{\@pyplot@positive@frac}{%
    1-\@pyplot@negative@frac}

  \coordinate (pyplot plotarea left) at ($(pyplot origin)+
  (-\@pyplot@negative@frac*\@pyplot@plotarea@x@size@padded,0)$);

  \coordinate (pyplot plotarea right) at ($(pyplot origin)+
  (\@pyplot@positive@frac*\@pyplot@plotarea@x@size@padded,0)$);

  \coordinate (pyplot axarea left) at ($(pyplot plotarea left)+
  (-\@pyplot@axarea@pad@left,0)$);

  \coordinate (pyplot axarea right) at ($(pyplot plotarea right)+
  (\@pyplot@axarea@pad@right,0)$);

  \path let
  \p1=(pyplot plotarea left),
  \p2=(pyplot plotarea right) in \pgfextra{
    \xdef\@pyplot@plotarea@tikz@xmin{\x1}
    \xdef\@pyplot@plotarea@tikz@xmax{\x2}
    \dimensionalize[unit=\@pyplot@unit]{\@pyplot@plotarea@tikz@xmin,
      \@pyplot@plotarea@tikz@xmax}
    \dimensionalize[unit=]{\@pyplot@plotarea@tikz@xmin,
      \@pyplot@plotarea@tikz@xmax}
  };

  \draw[pyplot axis] (pyplot axarea left) -- (pyplot axarea right)
  node[pos=0](pyplot x base){} node[pos=1](pyplot x tip){};

  % ..:: y-axis ::..

  \ifthenelse{\equal{\@pyplot@y@axis@draw@location}{center}}{
    \gdef\@pyplot@y@axis@draw@ref@point{pyplot origin}
  }{
    \gdef\@pyplot@y@axis@draw@ref@point{pyplot axarea left}
  }

  \def\@pyplot@plotarea@bottom@shift{-\@pyplot@negative@frac*
    \@pyplot@plotarea@y@size@padded}
  \ifthenelse{\equal{\@pyplot@x@axis@draw@location}{center}}{
    \pgfmathsetmacro{\@pyplot@negative@frac}{%
      (\@pyplot@plotarea@ycenter-\@pyplot@plotarea@ymin)/
      (\@pyplot@plotarea@ymax-\@pyplot@plotarea@ymin)}
    \pgfmathsetmacro{\@pyplot@positive@frac}{%
      1-\@pyplot@negative@frac}
  }{
    \pgfmathsetmacro{\@pyplot@negative@frac}{0}
    \pgfmathsetmacro{\@pyplot@positive@frac}{1}
    \edef\@pyplot@plotarea@bottom@shift{\@pyplot@plotarea@bottom@shift+
      \@pyplot@axarea@pad@bottom}
  }

  \coordinate (pyplot plotarea bottom) at
  ($(\@pyplot@y@axis@draw@ref@point)+(0,\@pyplot@plotarea@bottom@shift)$);

  \coordinate (pyplot plotarea top) at ($(\@pyplot@y@axis@draw@ref@point)+
  (0,\@pyplot@positive@frac*\@pyplot@plotarea@y@size@padded)$);

  \coordinate (pyplot axarea bottom) at ($(pyplot plotarea bottom)+
  (0,-\@pyplot@axarea@pad@bottom)$);

  \coordinate (pyplot axarea top) at ($(pyplot plotarea top)+
  (0,\@pyplot@axarea@pad@top)$);

  \path let
  \p1=(pyplot plotarea bottom),
  \p2=(pyplot plotarea top) in \pgfextra{
    \xdef\@pyplot@plotarea@tikz@ymin{\y1}
    \xdef\@pyplot@plotarea@tikz@ymax{\y2}
    \dimensionalize[unit=\@pyplot@unit]{\@pyplot@plotarea@tikz@ymin,
      \@pyplot@plotarea@tikz@ymax}
    \dimensionalize[unit=]{\@pyplot@plotarea@tikz@ymin,
      \@pyplot@plotarea@tikz@ymax}
  };

  \draw[pyplot axis] (pyplot axarea bottom) -- (pyplot axarea top)
  node[pos=0](pyplot y base){} node[pos=1](pyplot y tip){};

  % ..:: Other handy variables while we're here ::..

  \coordinate (pyplot plotarea bottom left) at
  (pyplot plotarea left|-pyplot plotarea bottom);

  \coordinate (pyplot plotarea top right) at
  (pyplot plotarea top-|pyplot plotarea right);

  \coordinate (pyplot axarea bottom left) at
  (pyplot axarea left|-pyplot axarea bottom);

  \coordinate (pyplot axarea top right) at
  (pyplot axarea top-|pyplot axarea right);

  \ifthenelse{\equal{\@pyplot@show@area@debug}{true}}{
    \draw[pyplot plot area debug]
    (pyplot plotarea bottom left) rectangle (pyplot plotarea top right);
    \draw[pyplot plot area debug]
    (pyplot axarea bottom left) rectangle (pyplot axarea top right);
  }{}

  \pyplot@generate@scaling@function
}

% Generate a command that produce node scaling to required text height
\newcommand{\pyplot@generate@scaling@function}{
  \coordinate (pyplot plotarea middle) at
  ($(pyplot plotarea bottom left)!0.5!(pyplot plotarea top right)$);

  \begin{scope}
    % Clip so that the invisible node doesn't take up any more space than
    % the actual plot
    \clip (pyplot plotarea bottom left) rectangle (pyplot plotarea top right);

    % Invisible normal font example label, just for its size
    \node (pyplot tmp) at (pyplot plotarea middle)
    {\phantom{$123$}};

    % Compute the scaling
    \path let
    \p1=(pyplot tmp.south),
    \p2=(pyplot tmp.north) in \pgfextra{
      \tikzmath{\@pyplot@internal@text@normal@height = \y2-\y1;}
      \dimensionalize[unit=\@pyplot@unit]{\@pyplot@internal@text@normal@height}
      \xdef\@pyplot@internal@text@normal@height{
        \@pyplot@internal@text@normal@height}
    };
  \end{scope}

  \def\pyplot@internal@compute@scaling##1{
    \tikzmath{\@pyplot@label@scale=##1\@pyplot@unit/
      \@pyplot@internal@text@normal@height;}
    \xdef\@pyplot@label@scale{\@pyplot@label@scale}
  }
}

% Add axis ticks
\define@key{@pyplot@keys}{axis}{\def\@pyplot@tick@axis{#1}}
\define@key{@pyplot@keys}{internal axis}{\def\@pyplot@tick@internal@axis{#1}}
\define@key{@pyplot@keys}{min}{\def\@pyplot@ticks@min{#1}}
\define@key{@pyplot@keys}{max}{\def\@pyplot@ticks@max{#1}}
\define@key{@pyplot@keys}{count}{\def\@pyplot@ticks@count{#1}}
\define@key{@pyplot@keys}{special}{\def\@pyplot@special@ticks{#1}}
\define@key{@pyplot@keys}{labels}{\def\@pyplot@tick@labels{#1}}
\define@key{@pyplot@keys}{tick size}{\def\@pyplot@ticks@size{#1}}
\define@key{@pyplot@keys}{label size}{\def\@pyplot@tick@label@size{#1}}
\define@key{@pyplot@keys}{label offset}{\def\@pyplot@tick@label@offset{#1}}
\define@key{@pyplot@keys}{format}{\def\@pyplot@label@format{#1}}
\define@key{@pyplot@keys}{contour}{\def\@pyplot@tick@contour{#1}}
% The main command to add ticks
\newcommand{\pyplot@add@ticks}[1]{
  \setkeys{@pyplot@keys}{axis=,#1}
  \pykzmathinline[@pyplot@num@ax]{len('\@pyplot@tick@axis')}
  \pgfmathparse{\@pyplot@num@ax>=1 ? 1 : 0}
  \ifthenelse{\pgfmathresult>0}{
    \foreach \@ax@i in {1,...,\@pyplot@num@ax} {
      \pykzmathinline[@pyplot@which@ax]{'\@pyplot@tick@axis'[\@ax@i-1]}
      \pyplot@internal@add@ticks{internal axis=\@pyplot@which@ax, #1}
    }
  }{}
}
% Internal command that gets called to draw the ticks
\newcommand{\pyplot@internal@add@ticks}[1]{
  % ..:: Select axis ::..
  \setkeys{@pyplot@keys}{internal axis=,#1}
  \ifthenelse{\equal{\@pyplot@tick@internal@axis}{}}{
    \PackageError{pyplot}{Unspecified axis}{Set axis=x or axis=y}
  }{}

  % ..:: Min and max values that ticks span ::..
  \ifthenelse{\equal{\@pyplot@tick@internal@axis}{x}}{
    \setkeys{@pyplot@keys}{min=\@pyplot@plotarea@xmin,#1}
    \setkeys{@pyplot@keys}{max=\@pyplot@plotarea@xmax,#1}
  }{
    \setkeys{@pyplot@keys}{min=\@pyplot@plotarea@ymin,#1}
    \setkeys{@pyplot@keys}{max=\@pyplot@plotarea@ymax,#1}
  }

  % ..:: Other parameters ::..
  \setkeys{@pyplot@keys}{count=2,#1}
  \setkeys{@pyplot@keys}{special=,#1}
  \setkeys{@pyplot@keys}{labels=,#1}
  \setkeys{@pyplot@keys}{tick size=0.06\@pyplot@unit,#1}
  \setkeys{@pyplot@keys}{label size=0.13,#1}
  \pyplot@internal@compute@scaling{\@pyplot@tick@label@size}
  \setkeys{@pyplot@keys}{label offset=0.1,#1}
  \setkeys{@pyplot@keys}{format=.2f,#1}
  \setkeys{@pyplot@keys}{contour=1pt,#1}

  % ..:: Save custom labels to list ::..
  \ifthenelse{\equal{\@pyplot@tick@labels}{}}{
    % Label directly using the tick value
    \makelist{pyplot@list}{\@pyplot@special@ticks}}{
    % Label using user-created tick labels
    \makelist{pyplot@list}{\@pyplot@tick@labels}}

  % ..:: Set the tick label formatter ::..
  \pykzexec{pyplot_label_fmt = lambda x: '{0:\@pyplot@label@format}'.format(x)}
  \xdef\@pyplot@format@function{pyplot_label_fmt}
  \pykzexec{import re;
    is_number = lambda s: not any([c.isalpha() for c in s])}

  % ..:: Generate ticks ::..
  \pykzexec{tick_list = np.array([])}
  \pgfmathparse{\@pyplot@ticks@count>0 ? 1 : 0}
  \ifthenelse{\pgfmathresult>0}{
    \foreach \@i in {1,...,\@pyplot@ticks@count} {
      \pykzexec{new_tick = (\@i-1)/(\@pyplot@ticks@count-1)*(
        \@pyplot@ticks@max-\@pyplot@ticks@min)+\@pyplot@ticks@min}
      \pykzexec{tick_list = np.append(tick_list, [new_tick])}
    }
  }{}
  \foreach \@special@tick in \@pyplot@special@ticks {
    \pykzexec{tick_list = np.append(tick_list, [\@special@tick])}
  }
  \pykzmathinline[@pyplot@num@ticks]{tick_list.size}

  % ..:: Plot ticks ::..
  \contourlength{\@pyplot@tick@contour}
  \foreach \@i in {1,...,\@pyplot@num@ticks} {

    % ..:: Draw the "tick" ::..
    \pykzmathinline[@pyplot@tick@value]{tick_list[\@i-1]}
    \ifthenelse{\equal{\@pyplot@tick@internal@axis}{x}}{
      \tikzmath{\@pyplot@tick@pos=\pyplot@internal@map@x{\@pyplot@tick@value};}
      \coordinate (tmp) at (\@pyplot@tick@pos, 0.0);
      \coordinate (pyplot tick pos) at (tmp|-pyplot origin);
      \draw[pyplot major tick] (pyplot tick pos) -- ++(0,-\@pyplot@ticks@size)
      node[pos=1](tick label coord){};
    }{
      \tikzmath{\@pyplot@tick@pos=\pyplot@internal@map@y{\@pyplot@tick@value};}
      \coordinate (tmp) at (0.0, \@pyplot@tick@pos);
      \coordinate (pyplot tick pos) at (tmp-|\@pyplot@y@axis@draw@ref@point);
      \draw[pyplot major tick] (pyplot tick pos) -- ++(-\@pyplot@ticks@size,0)
      node[pos=1](tick label coord){};
    }

    % ..:: Get tick label text (the number) ::..
    \pgfmathparse{\@i>\@pyplot@ticks@count ? 1:0}
    \def\pyplot@numerical@tick{True}
    \def\pyplot@special@tick{False}
    \ifthenelse{\pgfmathresult>0}{
      \def\pyplot@special@tick{True}
      \tikzmath{\@j=int(\@i-\@pyplot@ticks@count);}
      \edef\@pyplot@this@label{\list@nth{pyplot@list}{\@j}}
      \pykzmathinline[is@number]{is_number('\@pyplot@this@label')}
      \ifthenelse{\equal{\is@number}{True}}{
        \edef\@pyplot@tick@value{\list@nth{pyplot@list}{\@j}}
      }{
        \def\pyplot@numerical@tick{False}
        \def\@pyplot@tick@label{\list@nth{pyplot@list}{\@j}}
        \def\@pyplot@tick@label@abs{\@pyplot@tick@label}
      }
    }{}
    \ifthenelse{\equal{\pyplot@numerical@tick}{True}}{
      \ifthenelse{\equal{\pyplot@special@tick}{False}}{
        \pykzmathinline[@pyplot@tick@label]{
          \@pyplot@format@function(\@pyplot@tick@value)}
      }{
        % Do not format the user-defined "special" ticks
        \def\@pyplot@tick@label{\@pyplot@tick@value}
      }
      % Remove the minus sign for proper
      \pykzmathinline[@pyplot@tick@label@abs]{
        '\@pyplot@tick@label'[1:] if '\@pyplot@tick@label'[0]=='-' else
        \@pyplot@tick@label}
    }{}

    % ..:: Absolute-value tick label just for centering ::..
    \ifthenelse{\equal{\@pyplot@tick@internal@axis}{x}}{
      \def\@pyplot@internal@tick@label@phantom{\@pyplot@tick@label@abs}
      \def\@pyplot@internal@tick@label@anchor{north}
      \def\@pyplot@internal@tick@label@shift{
        0,-\@pyplot@tick@label@offset\@pyplot@unit}
    }{
      \def\@pyplot@internal@tick@label@phantom{\@pyplot@tick@label}
      \def\@pyplot@internal@tick@label@anchor{east}
      \def\@pyplot@internal@tick@label@shift{
        -\@pyplot@tick@label@offset\@pyplot@unit,0}
    }
    \node[pyplot major tick label,
    scale=\@pyplot@label@scale,
    anchor=\@pyplot@internal@tick@label@anchor,
    shift={(\@pyplot@internal@tick@label@shift)},
    opacity=0] (pyplot tick label) at (tick label coord)
    {\phantom{$\@pyplot@internal@tick@label@phantom$}};

    \begin{pgfonlayer}{pyplot fg}
      \node[pyplot major tick label,
      scale=\@pyplot@label@scale,
      anchor=north east] at (pyplot tick label.north east)
      {\contour{\@pyplot@background@color}{$\@pyplot@tick@label$}};
    \end{pgfonlayer}

  }
}

% Create axis label
\define@key{@pyplot@keys}{label}{\def\@pyplot@axis@label@text{#1}}
\define@key{@pyplot@keys}{anchor}{\def\@pyplot@axis@label@anchor{#1}}
\define@key{@pyplot@keys}{xshift}{\def\@pyplot@axis@label@xshift{#1}}
\define@key{@pyplot@keys}{yshift}{\def\@pyplot@axis@label@yshift{#1}}
\define@key{@pyplot@keys}{rotate}{\def\@pyplot@axis@label@rotate{#1}}
\newcommand{\pyplot@axis@label}[1]{
  \setkeys{@pyplot@keys}{axis=,#1}
  \ifthenelse{\equal{\@pyplot@tick@axis}{}}{
    \PackageError{pyplot}{Unspecified axis}{Set axis=x or axis=y}
  }{}

  \setkeys{@pyplot@keys}{label=,#1}

  \ifthenelse{\equal{\@pyplot@tick@axis}{x}}{
    \setkeys{@pyplot@keys}{anchor=south east,#1}
    \setkeys{@pyplot@keys}{xshift=0,#1}
    \setkeys{@pyplot@keys}{yshift=0.15,#1}
  }{
    \setkeys{@pyplot@keys}{anchor=north east,#1}
    \setkeys{@pyplot@keys}{xshift=-0.15,#1}
    \setkeys{@pyplot@keys}{yshift=0,#1}
  }

  \setkeys{@pyplot@keys}{rotate=0,#1}
  \setkeys{@pyplot@keys}{label size=0.18,#1}
  \pyplot@internal@compute@scaling{\@pyplot@tick@label@size}

  % Draw the label
  \def\@pyplot@tmp@tip{ tip}
  \node[pyplot axis label,
  anchor=\@pyplot@axis@label@anchor,
  scale=\@pyplot@label@scale,
  xshift=\@pyplot@axis@label@xshift\@pyplot@unit,
  yshift=\@pyplot@axis@label@yshift\@pyplot@unit]
  at (pyplot \@pyplot@tick@axis\@pyplot@tmp@tip)
  {\@pyplot@axis@label@text};
}

% Map x value from math to TikZ coordinates
\newcommand{\pyplot@internal@map@x}[1]{
  ((#1-\@pyplot@plotarea@xmin)/(\@pyplot@plotarea@xmax-\@pyplot@plotarea@xmin)*
  (\@pyplot@plotarea@tikz@xmax-\@pyplot@plotarea@tikz@xmin)+
  \@pyplot@plotarea@tikz@xmin)
}

% Map y value from math to TikZ coordinates
\newcommand{\pyplot@internal@map@y}[1]{
  ((#1-\@pyplot@plotarea@ymin)/(\@pyplot@plotarea@ymax-\@pyplot@plotarea@ymin)*
  (\@pyplot@plotarea@tikz@ymax-\@pyplot@plotarea@tikz@ymin)+
  \@pyplot@plotarea@tikz@ymin)
}

% Generate a linear range of N points from min to max
\newcommand{\pyplot@linrange}[4]{
  \def\@pyplot@linrange@name{#1}
  \def\@pyplot@linrange@min{#2}
  \def\@pyplot@linrange@max{#3}
  \def\@pyplot@linrange@N{#4}
  \pykzexec{\@pyplot@linrange@name=np.linspace(\@pyplot@linrange@min,
    \@pyplot@linrange@max,\@pyplot@linrange@N)}
}

% Map a function over an x-range to generate (x,y) data.
\newcommand{\pyplot@map}[3][]{
  \def\@pyplot@xy@data@name{#1}
  \def\@pyplot@x@data{#2}
  \def\@pyplot@function{#3}

  % Determine max stride
  \pykzmathinline[@pyplot@x@data@size]{len(\@pyplot@x@data)}
  \pykzmathinline[@pyplot@unit@strlen]{len('\@pyplot@unit')}

  \tikzmath{
    \@pyplot@map@stride = int(floor(\@pyplot@python@maxchar/(
    2*(9+\@pyplot@map@precision+\@pyplot@unit@strlen)+4)));
    \@pyplot@stride@steps = int(\@pyplot@x@data@size/\@pyplot@map@stride)+1;
  }

  \def\@pyplot@exp{e}
  \pykzexec{pyplot_inbounds = lambda x, y:
    (not \@pyplot@clip) or
    (x>=\@pyplot@plotarea@xmin and
    x<=\@pyplot@plotarea@xmax and
    y>=\@pyplot@plotarea@ymin and
    y<=\@pyplot@plotarea@ymax)}

  \def\@pyplot@xy@data{}
  \foreach \@i in {1,...,\@pyplot@stride@steps} {
    \pykzmathinline[pyplot@xy@batch]{
      ' '.join('({0:.\@pyplot@map@precision\@pyplot@exp}*1\@pyplot@unit,%
      {1:.\@pyplot@map@precision\@pyplot@exp}*1\@pyplot@unit)'.format(
      \pyplot@internal@map@x{_x},
      \pyplot@internal@map@y{\@pyplot@function(_x)}
      ) if pyplot_inbounds(_x, \@pyplot@function(_x)) else ''
      for _x in
      \@pyplot@x@data[(\@i-1)*\@pyplot@map@stride:min(\@i*\@pyplot@map@stride,
      \@pyplot@x@data@size)])}
    \xdef\@pyplot@xy@data{\@pyplot@xy@data \pyplot@xy@batch}
  }

  \ifthenelse{\equal{\@pyplot@xy@data@name}{}}{}{
    \expandafter\xdef\csname \@pyplot@xy@data@name\endcsname{\@pyplot@xy@data}}%
}

% Place a TikZ coordinate at a specific (x,y) location
\newcommand{\pyplot@point}[3][point]{
  \pykzexec{pyplot__tmp_x = [#2]}
  \pykzexec{pyplot__tmp_y = lambda x: #3}
  \pyplot@map[@pt]{pyplot__tmp_x}{pyplot__tmp_y}
  \node (pyplot__tmp_point) at \@pt {};
  \coordinate (#1) at (pyplot__tmp_point.center);
}

% Create a callable colormap object cmap(x)
\define@key{@pyplot@keys}{map}{\def\@pyplot@colormap@style{#1}}
\define@key{@pyplot@keys}{name}{\def\@pyplot@colormap@function@name{#1}}
\newcommand{\pyplot@colormap}[3][]{
  \setkeys{@pyplot@keys}{map=inferno,#1}
  \setkeys{@pyplot@keys}{name=@cmap,#1}
  \def\@pyplot@colormap@min{#2}
  \def\@pyplot@colormap@max{#3}
  \pykzexec{import matplotlib as mpl}
  \pykzexec{from matplotlib import pyplot as plt}
  \pykzexec{cmap_base = plt.get_cmap('\@pyplot@colormap@style')}
  \pykzexec{cmap_nrm = mpl.colors.Normalize(vmin=\@pyplot@colormap@min,
    vmax=\@pyplot@colormap@max)}
  \pykzexec{cmap_rgba = mpl.cm.ScalarMappable(norm=cmap_nrm, cmap=cmap_base)}
  \pykzexec{cmap = lambda x : ('{0}'.format(mpl.colors.to_hex(
    cmap_rgba.to_rgba(x))))[1:]}
  % Make a function which you can call to generate a new color
  \expandafter\newcommand\csname\@pyplot@colormap@function@name\endcsname[2][]{
    \pykzmathinline[@pyplot@colormap@clr]{cmap(##2)}
    \definecolor{##1}{HTML}{\@pyplot@colormap@clr}
  }
}

% Create a clipped plot area within which elemnts are not draw if they fall
% outside the plot area
\define@key{@pyplot@keys}{pad}{\def\@pyplot@clip@area@pad{#1}}
\define@key{@pyplot@keys}{leftpad}{\def\@pyplot@clip@area@pad@left{#1}}
\newenvironment{pyplot@plot@area}[1][]{%
  \setkeys{@pyplot@keys}{pad=0,#1}
  \setkeys{@pyplot@keys}{leftpad=-1,#1}
  \begin{scope}%
    % General clipping area (apply global padding)
    \coordinate (clip area bottom left) at
    ($(pyplot plotarea bottom left)+(-\@pyplot@clip@area@pad,
    -\@pyplot@clip@area@pad)$);
    \coordinate (clip area top right) at
    ($(pyplot plotarea top right)+(\@pyplot@clip@area@pad,
    \@pyplot@clip@area@pad)$);

    % Apply per-edge padding
    \pgfmathparse{\@pyplot@clip@area@pad@left<0 ? 1:0}
    \ifthenelse{\pgfmathresult>0}{}{
      \coordinate (clip area bottom left) at
      ($(clip area bottom left)+(\@pyplot@clip@area@pad-
      \@pyplot@clip@area@pad@left,0)$);
    }

    % Make clipping area
    \clip (clip area bottom left) rectangle (clip area top right);
  }{%
  \end{scope}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Private functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TODO

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/beamer.tex <==
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Colors ::..
\definecolor{beamerYellow}{HTML}{f1d46a}
\definecolor{beamerDarkYellow}{HTML}{bbb870}
\definecolor{beamerRed}{HTML}{db6245}
\definecolor{beamerBlue}{HTML}{356397}
\definecolor{beamerDarkBlue}{HTML}{26415d}
\definecolor{beamerGrey}{HTML}{acacac}
\definecolor{beamerGreen}{HTML}{5da9a1}
\definecolor{beamerBlack}{HTML}{000000}

\setbeamercolor{alerted text}{fg=beamerRed}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Links ::..
\hypersetup{colorlinks,
  linkcolor={beamerRed},
  citecolor={beamerGrey},
  urlcolor={beamerBlue}}

\newcommand{\beamcite}[1]{{\color{beamerGrey}\cite{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Font ::..
% Font size
\usepackage{scrextend}
\changefontsizes{8pt}

% Check and cross marks
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\goodmark}{{\color{beamerGreen}\cmark}}
\newcommand{\badmark}{{\color{beamerRed}\xmark}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Text highlighting ::..
% From answer: https://tex.stackexchange.com/a/7545/90535
\newlength{\hl@depth@ref}
\settodepth{\hl@depth@ref}{g}
\newlength{\hl@height@ref}
\settoheight{\hl@height@ref}{T}
\newlength{\hl@width}%
\newcommand{\beamerhighlight}[2][beamerYellow]%
{%
  \settowidth{\hl@width}{#2}%
  \colorbox{#1}%
  {%
    \raisebox{-\hl@depth@ref}%
    {%
      \parbox[b][\hl@height@ref+\hl@depth@ref][c]{\hl@width}{\centering#2}%
    }%
  }%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: TikZ elements ::..
% Hyperlinkable nodes
% from: https://tex.stackexchange.com/a/36111/90535
\tikzset{
  hyperlink node/.style={
    alias=sourcenode,
    append after command={
      let     \p1 = (sourcenode.north west),
      \p2=(sourcenode.south east),
      \n1={\x2-\x1},
      \n2={\y1-\y2} in
      node [inner sep=0pt, outer sep=0pt,anchor=north west,at=(\p1)]
      {\hyperlink{#1}{\XeTeXLinkBox{\phantom{\rule{\n1}{\n2}}}}}
    }
  }
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Footer: progress bar and sections list ::..
\setbeamertemplate{navigation symbols}{}
% >> Progress variables <<
\newcommand{\slidefooter}[1]{
  \def\slidefooter@text{#1}
}
\def\footer@text@xshift{1mm}
\def\pagecounter@top{}
% >> Section list variables <<
\def\short@section{}
\def\beamer@sections{}
\def\saved@beamer@sections{}
\def\beamer@appendices{}
\def\saved@beamer@appendices{}
\def\appendix@started{false}
\def\appendix@start@slide{}
\def\saved@appendix@start@slide{-1}
\newcommand{\beamersection}[2][]{
  % Add a new section to the slides
  \pykzexec{options='#1'.split(',')}
  \pykzmathinline[is@appendix]{'true' if 'appendix' in options else 'false'}
  \pykzmathinline[short@section]{''.join(s for s in options if s!='appendix')}
  \ifthenelse{\equal{\short@section}{}}{
    \xdef\short@section{#2}
  }{}
  \ifthenelse{\equal{\is@appendix}{false} \AND \equal{\appendix@started}{true}}{
    \PackageError{beamer}{Cannot have non-appendix sections after appendix has
      started}{Include the appendix optional argument}
  }{
    \ifthenelse{\equal{\is@appendix}{true} \AND \equal{\appendix@started}{false}}{
      % Sets the state of the presentation into appendix mode
      \xdef\appendix@start@slide{\insertframenumber}
      \xdef\appendix@started{true}
      % Create an appendix demarcation slide
      \begin{frame}
        \tikzset{
          appendix text/.style={}
        }
        \begin{beamertikzpicture}
          \getframecoord{0,0}
          \node[appendix text] at (\framecoord) {%
            \beamerhighlight[beamerDarkBlue]{\color{white}Appendices}};
        \end{beamertikzpicture}
      \end{frame}
    }{}
  }
  \section{#2}
  % Add to list of all sections
  \ifthenelse{\equal{\appendix@started}{false}}{
    \tikzmath{
      \current@slide@number = \insertframenumber;
    }
    \xdef\@variable{beamer@sections}
  }{
    \tikzmath{
      \current@slide@number = int(\insertframenumber-\appendix@start@slide);
    }
    \xdef\@variable{beamer@appendices}
  }
  \ifthenelse{\equal{\csname \@variable\endcsname}{}}{
    \expandafter\xdef\csname \@variable\endcsname{
      \short@section/\current@slide@number}
  }{
    \expandafter\xdef\csname \@variable\endcsname{
      \short@section/\current@slide@number,\csname \@variable\endcsname}
  }
}
%%%%%%%%%%%%%%%%%
% Make the footer
%%%%%%%%%%%%%%%%%
\newcommand{\get@section@color}[1]{\pykzmathinline[this@section@color]{
    section_color_wheel[\section@counter-(\section@counter//n_section_colors)*n_section_colors]}}
\newcommand{\load@aux}{
  % >> Load sections from aux file <<
  \ifthenelse{\equal{\insertframenumber}{1}}{
    % Load sections
    \pykzexec{f = open('../../beamersections.aux','r')}
    \pykzexec{raw_sections = f.read()}
    \pykzexec{sections = raw_sections.split(',')}
    \pykzmathinline[saved@beamer@sections]{raw_sections}
    \pykzexec{f.close()}

    % Load appendices
    \pykzexec{f = open('../../beamerappendices.aux','r')}
    \pykzexec{raw_appendices = f.read()}
    \pykzexec{appendices = raw_appendices.split(',')}
    \pykzmathinline[saved@beamer@appendices]{raw_appendices}
    \pykzexec{f.close()}
    \pykzexec{f = open('../../appendixstart.aux','r')}
    \pykzmathinline[saved@appendix@start@slide]{f.read()}
    \pykzexec{f.close()}
  }{}
}
\setbeamertemplate{footline}{
  \load@aux

  % >> Write sections to aux file <<
  \ifthenelse{\equal{\insertframenumber}{\inserttotalframenumber}}{
    % Write sections
    \pykzexec{f = open('../../beamersections.aux','w')}
    \pykzexec{print('\beamer@sections',file=f,end='')}
    \pykzexec{f.close()}

    % Write appendices
    \pykzexec{f = open('../../beamerappendices.aux','w')}
    \pykzexec{print('\beamer@appendices',file=f,end='')}
    \pykzexec{f.close()}
    \pykzexec{f = open('../../appendixstart.aux','w')}
    \ifthenelse{\equal{\appendix@start@slide}{}}{
      \pykzexec{print('\inserttotalframenumber',file=f,end='')}
    }{
      \pykzexec{print('\appendix@start@slide',file=f,end='')}
    }
    \pykzexec{f.close()}
  }{}

  % >> TikZ styles <<
  \tikzset{
    every node/.append style= {
      inner sep=0,
      outer sep=0
    },
    progress line/.style = {
      draw=black,
      line width=0.15mm
    },
    appendix line/.style={
      dashed
    },
    progress tip/.style = {
      circle,
      draw=black,
      fill=black,
      minimum size=1mm
    },
    section checkpoint/.style={
      circle,
      draw=##1!70,
      fill=##1!30,
      line width=0.2mm,
      minimum size=1.4mm
    },
    page counter/.style = {
      anchor=south east
    },
    footer text/.style = {
      anchor=south west,
      align=left,
      scale=0.8
    },
    section color bubble/.style = {
      circle,
      inner sep=0,
      outer sep=0.2mm,
      minimum size=0.5mm,
      fill=##1
    }
  }

  % >> Progress bar <<
  \def\progressline@xpad@west{1mm}
  \def\progressline@xpad@east{2mm}
  \def\footer@text@yshift{1mm}
  \pgfdeclarelayer{bg}
  \pgfsetlayers{bg,main}
  \begin{tikzpicture}[overlay,remember picture,shift={(current page.south west)}]
    %
    % @ Footer text @
    \node[footer text] (text)
    at (\footer@text@xshift,\footer@text@yshift)
    {\slidefooter@text};
    \path let \p1=(text.east) in \pgfextra{
      \xdef\progressline@x{\x1}
      \xdef\left@lim{\x1}
    };
    % @ Page counter @
    \ifthenelse{\equal{\appendix@started}{false}}{
      \tikzmath{
        \current@slide@number = \insertframenumber;
        \total@slide@number = \saved@appendix@start@slide;
      }
    }{
      \tikzmath{
        \current@slide@number = int(\insertframenumber-\saved@appendix@start@slide);
        \total@slide@number = int(\inserttotalframenumber-\saved@appendix@start@slide);
      }
    }
    \node[page counter] (counter) at
    ($(current page.south east)+(-\footer@text@xshift,\footer@text@yshift)$)
    {\current@slide@number/\total@slide@number};
    \path let
    \p1=(counter.east),
    \p2=(counter.north) in \pgfextra{
      \xdef\progressline@y{\y1}
      \xdef\right@lim{\x1-5mm}
      \xdef\pagecounter@top{\y2}
    };
    % @ Section checkpoints @
    \pykzexec{section_color_wheel=['beamerGreen','beamerBlue','beamerYellow','beamerRed'];
      n_section_colors=len(section_color_wheel)}
    \tikzmath{
      \width = \right@lim-\left@lim-\progressline@xpad@west-\progressline@xpad@east;
    }
    \coordinate (progress line start) at
    (\progressline@x+\progressline@xpad@west,\progressline@y);
    \def\section@counter{0}
    \ifthenelse{\equal{\appendix@started}{false}}{
      \xdef\saved@sections{\saved@beamer@sections}
    }{
      \xdef\saved@sections{\saved@beamer@appendices}
    }
    \foreach \section/\section@page in \saved@sections {
      \tikzmath{
        \progress = (\section@page+1)/\total@slide@number*\width;
      }
      \get@section@color{\section@counter}
      \node[section checkpoint=\this@section@color,
      hyperlink node=\section] at
      ($(progress line start)+(\progress*1pt,0)$) {};
      \counter@increment{\section@counter}
    }
    % @ Progress line @
    \tikzmath{
      \progress = \current@slide@number/\total@slide@number*\width;
    }
    \begin{pgfonlayer}{bg}
      \ifthenelse{\equal{\appendix@started}{false}}{
        \draw[progress line] (progress line start) -- ++(\progress*1pt,0) node(tip){};
      }{
        \draw[progress line,appendix line] (progress line start) --
        ++(\progress*1pt,0) node(tip){};
      }
    \end{pgfonlayer}
    \node[progress tip] at (tip) {};
  \end{tikzpicture}

  % >> Section list <<
  \def\list@begin@yshift{0.7em}
  \def\list@dy{1em}
  \begin{tikzpicture}[overlay,remember picture,shift={(current page.south east)}]
    \tikzset{
      sections list element/.style={
        anchor=east,
        scale=0.8
      }
    }
    \def\section@counter{0}
    \ifthenelse{\equal{\appendix@started}{false}}{
      \xdef\saved@sections{\saved@beamer@sections}
      \xdef\@variable{sections}
    }{
      \xdef\saved@sections{\saved@beamer@appendices}
      \xdef\@variable{appendices}
    }
    \foreach \section/\section@page in \saved@sections {
      \tikzmath{
        \current@y = \pagecounter@top+\list@begin@yshift+\section@counter*\list@dy;
      }
      \ifthenelse{\equal{\short@section}{}}{
        \xdef\this@section{0}
      }{
        \pykzmathinline[this@section]{['\short@section' in section
          for section in \@variable].index(True)+1}
      }
      \pgfmathparse{\this@section==\section@counter+1 ? 1:0}
      \ifthenelse{\pgfmathresult>0}{
        \xdef\sectioncolor{beamerRed}
      }{
        \xdef\sectioncolor{beamerGrey}
      }
      \node[sections list element,
      color=\sectioncolor] (section text) at
      (-\footer@text@xshift,\current@y*1pt) {%
        \hyperlink{\section}{\color{\sectioncolor}\section}};
      \get@section@color{\section@counter}
      \node[section color bubble=\this@section@color,
      anchor=west] at (section text.east) {};
      \counter@increment{\section@counter}
    }
  \end{tikzpicture}

}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Hyperlinks to slides ::..
\setbeamertemplate{headline}{
  \load@aux
  \ifthenelse{\equal{\short@section}{}}{}{
    \ifthenelse{\equal{\appendix@started}{false}}{
      \xdef\@variable{sections}
    }{
      \xdef\@variable{appendices}
    }
    \pykzexec{start_page = int(\@variable[['\short@section' in section
      for section in \@variable].index(True)].split('/')[1])+1}
    \ifthenelse{\equal{\appendix@started}{false}}{
      \tikzmath{
        \current@slide@number = \insertframenumber;
      }
    }{
      \tikzmath{
        \current@slide@number = int(\insertframenumber-\saved@appendix@start@slide);
      }
    }
    \pykzexec{is_start = start_page==\current@slide@number}
    \pykzmathinline[is@start]{'true' if is_start else 'false'}
    \ifthenelse{\equal{\is@start}{true}}{
      \hypertarget{\short@section}{}
    }{}
  }
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Slides title ::..
\setbeamercolor{frametitle}{fg=black}
\setbeamerfont{frametitle}{size=\LARGE}
\setbeamertemplate{frametitle}{
  \def\frametitle@yshift{-5mm}
  \tikzset{
    frametitle style/.style={
      scale = 0.8,
      yshift = \frametitle@yshift,
      font = \bfseries
    }
  }
  \begin{tikzpicture}[overlay,remember picture,shift={(current page.north)}]
    \node[frametitle style] at (0,0) {\insertframetitle};
  \end{tikzpicture}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Page placement ::..
\def\slide@pad@sw{3mm,3mm}
\def\slide@pad@ne{3mm,3mm}
\newcommand{\getframecoord}[2][]{
  % Get absolute coordinate on slide, from fractional coordinate
  % Note that to make sense, the tikzpicture must be shifted to
  % (current page.south west)
  \xdef\frame@count{0}
  \foreach \val in {#2} {
    \pgfmathparse{\frame@count==0 ? 1:0}
    \ifthenelse{\pgfmathresult>0}{
      \xdef\c@x{\val}
    }{
      \xdef\c@y{\val}
    }
    \counter@increment{\frame@count}
  }
  \tikzmath{
    \Lx = \paperwidth/2;
    \Ly = \paperheight/2;
    \@x = \Lx*(1+\c@x);
    \@y = \Ly*(1+\c@y);
  }
  \xdef\framecoord{\@x*1pt,\@y*1pt}
  \ifthenelse{\equal{#1}{}}{}{\expandafter\xdef\csname #1\endcsname{\framecoord}}%
}
\newcommand{\placecursor}[2][cursor]{
  \getframecoord[@beamer@tmp@cursor@coord]{#2}
  \coordinate (#1) at (\@beamer@tmp@cursor@coord);
}
\newcommand{\beamergridoverlay}{
  % Overlay a grid to aid in element placement
  \begin{tikzpicture}[overlay,remember picture,shift={(current page.south west)}]
    \def\grid@dx{0.2}
    \def\grid@dy{0.2}
    \tikzmath{
      \x@next = -1+\grid@dx;
      \y@next = -1+\grid@dx;
    }
    \tikzset{
      grid line/.style={
        draw = black!30,
        line width=0.1mm,
        opacity=0.5
      },
      axis tick label/.style={
        text = black!30,
        fill = white,
        inner sep=0.5mm,
        scale = 0.8
      }
    }
    % X lines
    \foreach \x in {-1,\x@next,...,1} {
      \getframecoord[coord@bottom]{\x,-1}
      \pgfmathparse{abs(\x)<1e-3 ? 1:0}
      \ifthenelse{\pgfmathresult>0}{
        \draw[grid line,dashed] (\coord@bottom) -- ++(0,\paperheight);
      }{
        \draw[grid line] (\coord@bottom) -- ++(0,\paperheight);
      }
    }
    % Y lines
    \foreach \y in {-1,\y@next,...,1} {
      \getframecoord[coord@bottom]{-1,\y}
      \pgfmathparse{abs(\y)<1e-3 ? 1:0}
      \ifthenelse{\pgfmathresult>0}{
        \draw[grid line,dashed] (\coord@bottom) -- ++(\paperwidth,0);
      }{
        \draw[grid line] (\coord@bottom) -- ++(\paperwidth,0);
      }
    }
    % X labels
    \foreach \x in {-1,\x@next,...,1} {
      \pgfmathparse{abs(\x)>1e-3 && abs(\x)<1-1e-3 ? 1 : 0}
      \ifthenelse{\pgfmathresult>0}{
        \getframecoord[coord@bottom]{\x,0}
        \pgfmathprintnumberto[precision=2]{\x}{\x@rounded}
        \node[axis tick label] at (\coord@bottom) {\x@rounded};
      }{}
    }
    % Y labels
    \foreach \y in {-1,\x@next,...,1} {
      \pgfmathparse{abs(\y)>1e-3 && abs(\y)<1-1e-3 ? 1 : 0}
      \ifthenelse{\pgfmathresult>0}{
        \getframecoord[coord@bottom]{0,\y}
        \pgfmathprintnumberto[precision=2]{\y}{\y@rounded}
        \node[axis tick label] at (\coord@bottom) {\y@rounded};
      }{}
    }
  \end{tikzpicture}
}
\let\beamergrid\beamergridoverlay
\let\placegrid\beamergridoverlay
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Default TikZ environment ::..
\newenvironment{beamertikzpicture}[1][]{%
  \tikzset{%
    apply style/.code={%
      \tikzset{#1}%
    }%
  }%
  \begin{tikzpicture}[overlay,
    remember picture,
    shift={(current page.south west)},
    apply style/.expand once=#1]
  }{
  \end{tikzpicture}
}
\let\beamertikz\beamertikzpicture
\let\endbeamertikz\endbeamertikzpicture
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Itemize bullets ::..
\tikzset{
  beamer bullet point/.style={
    circle,
    fill=#1,
    minimum size=0.35em
  }
}
\def\item@y@offset{0.3em}
\foreach \@name/\@color in {
  one/beamerDarkBlue,two/beamerBlue,three/beamerGreen} {
  \expandafter\newsavebox\csname bullet@\@name\endcsname
  \begin{lrbox}{\csname bullet@\@name\endcsname}
    \begin{tikzpicture}[inner sep=0,outer sep=0,minimum size=0]
      \node at (0,0) {};
      \node[beamer bullet point=\@color] at (0,\item@y@offset) {};
    \end{tikzpicture}
  \end{lrbox}
  \global
  \expandafter\setbox\csname bullet@\@name\endcsname
  \expandafter\box\csname bullet@\@name\endcsname
}
\setlist[itemize,1]{label={\usebox\bullet@one}}
\setlist[itemize,2]{label={\usebox\bullet@two}}
\setlist[itemize,3]{label={\usebox\bullet@three}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ..:: Bibliography printing ::..
\setbeamertemplate{bibliography item}{\insertbiblabel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latex_common/book_style.tex <==
% No paragraph indentation
\setlength\parindent{1em}

% Paragraph spacing
\setlength{\parskip}{0pt}

\def\PtUnit{pt}

\def\innerSep{7cm}
\def\outerSep{1.5cm}
\def\topSep{2cm}
\def\botSep{2cm}
\def\chapterTopSep{2*\topSep}
\def\chapterBotMargin{2cm}

\tikzmath{
  \sidebarWidth = 0.9*\innerSep;
  \textMarginWidth = \innerSep-\sidebarWidth;
  \sidebarPad = 0.5cm;
  \topLabelSep = 2mm;
  \figureWidthLoc = \sidebarWidth-2*\sidebarPad;
}

\def\figureWidth{\figureWidthLoc\PtUnit}
\def\textMarginWidthUnits{\textMarginWidth\PtUnit}

% Expensive figure blocker
\xdef\bookCompileFigures{true}
\newcommand{\makeFigureToggled}[2][]{%
  \ifthenelse{\equal{\bookCompileFigures}{true}}{%
    #2%
  }{%
    \ifthenelse{\equal{#1}{}}{}{%
      \includegraphics[width=#1]{example-image-a}% 
    }{%
      \includegraphics[width=5cm]{example-image-a}%
    }%
  }%
}
\newcommand{\bookToggleFigures}{
  \ifthenelse{\equal{\bookCompileFigures}{true}}{
    \xdef\bookCompileFigures{false}
  }{
    \xdef\bookCompileFigures{true}
  }
}

% Colors
\definecolor{maroon}{rgb}{0.5, 0.0, 0.0}
\newcommand{\highlightcolor}{maroon}
\newcommand{\bookHighlight}[1]{{\itshape\color{\highlightcolor}#1}}
\xdef\sidebarColorNormal{black!10}

% Page types:
%  toc = table of contents
%  text = body text
%  biblio = references list
%  nom = nomenclature
\xdef\sectionType{text}

\usepackage[
% paperwidth=6in,
% paperheight=9in,
letterpaper,
inner=\innerSep,
outer=\outerSep,
top=\topSep,
bottom=\botSep]{geometry}

\pagestyle{fancy}

\fancyhf{} % clear header and footer
\renewcommand{\headrulewidth}{0pt} % no top line

% Figure caption style
\captionsetup[figure]{labelfont={sc},labelformat={default},labelsep=period,name={Figure}}

% Chapter, section, etc. names
\newcommand{\sectiontitle}{}
\newcommand{\setsectiontitle}[1]{\renewcommand{\sectiontitle}{#1}}
\newcommand{\invisiblesection}[1]{%
  \phantomsection%
  \stepcounter{section}%
  \addcontentsline{toc}{section}{\protect\numberline{\thesection}#1}%
}
\newcommand{\mySection}[2][visible]{
  \xdef\theSectionName{#2}
  \label{chapter:\thechapter}
  \ifthenelse{\equal{#1}{invisible}}{
    \invisiblesection{\theSectionName}
  }{
    \section{\theSectionName}
  }
  \label{section:\thesection}
}
\xdef\ChapterQuote{}
\newcommand{\myChapter}[3][]{
  \newpage
  \xdef\ChapterQuote{#1}
  \xdef\sectionType{text}
  \xdef\theChapterName{#2}
  \xdef\theSectionName{#3}
  \chapter{\theChapterName}
  \label{chapter:\thechapter}
  \mySection[invisible]{\theSectionName}
  % Reset counters
  \setcounter{Booktheorem}{0}
  \setcounter{Bookdefinition}{0}
  \setcounter{Bookcorollary}{0}
  \setcounter{Booklemma}{0}
  \setcounter{Bookproposition}{0}
  \setcounter{Bookcondition}{0}
  \setcounter{Bookassumption}{0}
  \setcounter{Bookexample}{0}
  % \expandafter\newsavebox\csname ChapterQuote\thechapter\endcsname
  % \begin{lrbox}{\csname ChapterQuote\thechapter\endcsname}
  %   #1
  % \end{lrbox}
}
\NewEnviron{bookAbstract}[1][]{
  \xdef\ChapterQuote{#1}
  \xdef\sectionType{abstract}
  \newpage
  \thispagestyle{plain}
  \xdef\theChapterName{Abstract}
  \chapter{\theChapterName}
  \label{chapter:\thechapter}
  \BODY
  \newpage
}
\newcommand{\myTOC}{
  \xdef\sectionType{toc}
  \tableofcontents
  \thispagestyle{plain}
  \newpage
}
\newcommand{\myLOF}{
  \xdef\sectionType{lof}
  \listoffigures
  \thispagestyle{plain}
  \newpage
}
\newcommand{\myLOT}{
  \xdef\sectionType{lot}
  \listoftables
  \thispagestyle{plain}
  \newpage
}
\newcommand{\myNomenclature}{
  \xdef\sectionType{nom}
  \printnomenclature
  \thispagestyle{plain}
  \newpage
}
\newcommand{\myBib}[1]{
  \xdef\sectionType{biblio}
  \bibliography{#1.bib}
}
\newcommand{\myBlankPage}{
  \null
  \thispagestyle{empty}%
  \addtocounter{page}{-1}%
  \begin{tikzpicture}[remember picture,overlay,shift={(current page.center)}]
    \node at (0,0) {-- This page is intentionally left blank. --};
  \end{tikzpicture}
  \newpage
}

\newcommand{\calcWidth}[1]{\tikzmath{\width=#1*\figureWidth;}%
  \xdef\customFigureWidth{\width\PtUnit}%
}

% \titlespacing*{\chapter}{0pt}{*0}{0pt}
\newlength{\HugeLetterHeight}
\newlength{\NormalLetterHeight}
\settoheight{\HugeLetterHeight}{\normalfont\Huge A}
\settoheight{\NormalLetterHeight}{A}
\tikzmath{
  \ChapterHeightText=-(\HugeLetterHeight+\parskip+\baselineskip-\NormalLetterHeight);
}
\xdef\ChapterHeightText{\ChapterHeightText\PtUnit}
\titleformat{\chapter}
{\normalfont\huge}
{}
{0cm}
{%
  \xdef\IsChapterPage{true}%
  \begin{tikzpicture}[remember picture,overlay,shift=(current page.north)]%
    \tikzset{
      chapter rule/.style={
        black,
        line width=1mm
      },
      every node/.append style={
        inner sep=0,
        outer sep=0
      },
      text node/.append style={
        anchor=north west,
        font={\bfseries},
        text width=\paperwidth-2*\outerSep
      }
    }
    \tikzmath{
      \ruleWidth = \paperwidth-2*\outerSep;
      \chapterHeight = 0.6cm;
    }
    \tikzmath{
      \xloc=-\paperwidth/2+\outerSep;
      \yloc=-\chapterTopSep;
    }
    \draw[chapter rule] (\xloc*1pt,\yloc*1pt) node(top rule){} to ++(\ruleWidth*1pt,0);
    \ifthenelse{\equal{\sectionType}{text}}{
      \node[text node,align=left] (chapter title)
      at ($(top rule.west)+(0,-\chapterHeight*1pt)$)
      {\thechapter\hspace{1cm} \theChapterName};
      \node[text node,text width=\paperwidth-2*\outerSep,
      anchor=north west,align=right] (first section title)
      at ($(chapter title.south west)+(0,-\chapterHeight*1pt)$)
      {\theSectionName};
      \coordinate (bottom rule start) at (first section title.west);
    }{
      \node[text node,align=left] (chapter title)
      at ($(top rule.west)+(0,-\chapterHeight*1pt)$)
      {\ifthenelse{\equal{\sectionType}{abstract}}{%
          Abstract%
        }{%
          \ifthenelse{\equal{\sectionType}{toc}}{%
            Table of Contents%
          }{%
            \ifthenelse{\equal{\sectionType}{lof}}{%
              List of Figures%
            }{%
              \ifthenelse{\equal{\sectionType}{lot}}{%
                List of Tables%
              }{%
                \ifthenelse{\equal{\sectionType}{biblio}}{%
                  Bibliography%
                }{%
                  Nomenclature%
                }%
              }%
            }%
          }%
        }%
      };
      \coordinate (bottom rule start) at (chapter title.west);
    }
    \ifthenelse{\equal{\ChapterQuote}{}}{}{
      \tikzset{
        chapter quote/.append style={
          align=left,
          font={\large\itshape},
          anchor=north west,
          text width=10cm
        }
      }
      \ifthenelse{\equal{\sectionType}{text}}{
        \node[chapter quote] (chapter quote node) at
        (first section title.north west) {\ChapterQuote};
        \path let
        \p1 = (chapter quote node.south west),
        \p2 = (first section title.south west)
        in \pgfextra{
          \tikzmath{
            \botlinexpos = \x1;
            \botlineypos = min(\y1,\y2);
          }
          \coordinate (bottom rule start) at (\botlinexpos*1pt,\botlineypos*1pt);
        };
      }{
        \node[chapter quote,yshift=-\chapterHeight*1pt] (chapter quote node) at
        (chapter title.south west) {\ChapterQuote};
        \coordinate (bottom rule start) at (chapter quote node.south west);
      }
      \xdef\ChapterQuote{}
    }
    \draw[chapter rule]
    ($(bottom rule start)+(0,-\chapterHeight*1pt)$)
    node(bottom rule){} to ++(\ruleWidth*1pt,0);
    \path let
    \p1=(top rule),
    \p2=(bottom rule)
    in \pgfextra{
      \tikzmath{
        \chapterHeadingHeight=\y1-\y2;
      }
      \xdef\chapterHeadingHeight{\chapterHeadingHeight\PtUnit}
    };
  \end{tikzpicture}%
  \tikzmath{%
    \ExtraSkip = (\chapterTopSep-\topSep)*1pt;%
    \TotalSkip = \ChapterHeightText+\ExtraSkip+\chapterHeadingHeight+%
    \chapterBotMargin;%
  }%
  \xdef\TotalSkip{\TotalSkip\PtUnit}%
  \vspace{\TotalSkip}%
}
\tikzmath{\ChapterHeight=\HugeLetterHeight+\parskip;}
\xdef\ChapterHeight{\ChapterHeight\PtUnit}
\titlespacing{\chapter}{0pt}{-\ChapterHeight}{*0}

\renewcommand{\sectionmark}[1]{\markboth{}{\thesection}}
\newcommand{\mySidebar}[2]{
  % #1: which page? LE, RO
  % #2: which style? plain, fancy
  \ifthenelse{\equal{#1}{LO}}{
    \def\sidebarLocation{north west}
  }{
    \def\sidebarLocation{north east}
  }
  \begin{tikzpicture}[
    remember picture,
    overlay,
    shift={(current page.\sidebarLocation)}
    ]
    \ifthenelse{\equal{#2}{plain}}{
      \def\sidebarColor{white}
    }{
      \def\sidebarColor{\sidebarColorNormal}
    }
    \tikzset{
      sidebar/.style={
        rectangle,
        anchor=\sidebarLocation,
        inner sep=0,
        outer sep=0,
        fill=\sidebarColor,
        minimum width=\sidebarWidth,
        minimum height=\paperheight
      },
      section line/.style={
        black,
        line width=0.3mm
      }
    }
    \node[sidebar] (sidebar region) at (0,0) {};
    % Chapter, section
    \ifthenelse{\equal{#2}{fancy}}{
      \ifthenelse{\equal{#1}{LO}}{
        \def\Pos{1}
        \def\Anchor{north east}
        \def\Align{right}
      }{
        \def\Pos{0}
        \def\Anchor{north west}
        \def\Align{left}
      }
      \draw[section line]
      ($(sidebar region.north west)+(\sidebarPad*1pt,-\topSep)$)
      to
      node[pos=\Pos,anchor=\Anchor,
      text width={\sidebarWidth-2*\sidebarPad},
      align=\Align,
      inner sep=0,
      outer sep=0,
      yshift=-\topLabelSep]
      (section label)
      {\Large%
        \ifthenelse{\equal{\sectionType}{toc}}{%
          {\itshape Contents}%
        }{%
          \ifthenelse{\equal{\sectionType}{biblio}}{%
            {\itshape Bibliography}%
          }{%
            \ifthenelse{\equal{\sectionType}{text}}{%
              \ifthenelse{\equal{#1}{LO}}{%
                \ifthenelse{\equal{\thechapter}{0}}{}{%
                  {\bfseries Chapter~\thechapter}\\%
                  {\itshape \theChapterName}%
                }%
              }{%
                {\bfseries Section~\rightmark}\\%
                {\itshape \theSectionName}%
              }%
            }{}%
          }
        }%
      }
      ($(sidebar region.north east)+(-\sidebarPad*1pt,-\topSep)$);
      \path let
      \p1=(section label.north),
      \p2=(section label.south)
      in \pgfextra{
        \tikzmath{
          \sidebarSectionLabelHeight=\y1-\y2;
        }
        \xdef\sidebarSectionLabelHeight{\sidebarSectionLabelHeight\PtUnit}
      };
    }{\xdef\sidebarSectionLabelHeight{0\PtUnit}}
    % Page number
    \ifthenelse{\equal{#1}{LO}}{
      \coordinate (page left) at
      ($(sidebar region.south west)+(\sidebarWidth/2*1pt,\botSep)$);
      \coordinate (page right) at
      ($(sidebar region.south east)+(-\sidebarPad*1pt,\botSep)$);
      \def\anchorPoint{north east}
    }{
      \coordinate (page left) at
      ($(sidebar region.south east)+(-\sidebarWidth/2*1pt,\botSep)$);
      \coordinate (page right) at
      ($(sidebar region.south west)+(\sidebarPad*1pt,\botSep)$);
      \def\anchorPoint{north west}
    }
    \draw[section line]
    (page left)
    to
    node[pos=1,
    anchor=\anchorPoint,
    inner sep=0,
    outer sep=0,
    yshift=-\topLabelSep,
    align=right
    ]{\thepage}
    (page right);
  \end{tikzpicture}
  % >>>>>>> Draw sidebar figures in the list
  \tikzset{
    figure/.append style={
      inner sep=0,
      outer sep=0,
      anchor=north
    }
  }
  % Define starting Y location
  \ifthenelse{\equal{\IsChapterPage}{true}}{
    \xdef\IsChapterPage{false}
    \tikzmath{
      \SidebarFigureYStart=-(\chapterTopSep+\chapterHeadingHeight+
      \chapterBotMargin);
    }
  }{
    \tikzmath{
      \SidebarFigureYStart=-(\topSep+\sidebarSectionLabelHeight+\SidebarFigureVPadding);
    }
  }
  \xdef\SidebarFigureY{\SidebarFigureYStart\PtUnit}
  % Loop through list of figures that are to be drawn
  \xdef\NewSidebarFigureList{}
  \xdef\Overflow{false}
  \foreach \figure in \SidebarContentList {
    \ifthenelse{\equal{\Overflow}{true}}{
      \AddToList{\NewSidebarFigureList}{\figure}
    }{
      \begin{tikzpicture}[
        remember picture,
        overlay,
        shift={(current page.\sidebarLocation)}
        ]
        \ifthenelse{\equal{#1}{LO}}{
          \tikzmath{\XLoc = \sidebarWidth/2;}
        }{
          \tikzmath{\XLoc = -\sidebarWidth/2;}
        }
        % Draw figure
        \edef\GetBox{\expandafter\usebox\csname \figure\endcsname}
        \node[figure,draw=none,opacity=0] (figure body phantom)
        at (\XLoc*1pt,\SidebarFigureY*1pt) {\phantom{\GetBox}};
        \path let
        \p1=(figure body phantom.north),
        \p2=(figure body phantom.south)
        in \pgfextra{
          \tikzmath{
            \height=(\y1-\y2);
            \SidebarFigureYBottom=\SidebarFigureY-\height;
          }
          \xdef\SidebarFigureYBottom{\SidebarFigureYBottom\PtUnit}
        };
        \pgfmathparse{\SidebarFigureYBottom>\SidebarFigureYEnd ? 1:0}
        \ifthenelse{\pgfmathresult>0}{
          \node[figure] (figure body) at (\XLoc*1pt,\SidebarFigureY*1pt)
          {\GetBox};
        }{
          \AddToList{\NewSidebarFigureList}{\figure}
          \xdef\Overflow{true}
        }
        \path let
        \p1=(figure body.north),
        \p2=(figure body.south)
        in \pgfextra{
          \tikzmath{\height=(\y1-\y2);}
          % Update Y
          \tikzmath{\SidebarFigureY=\SidebarFigureY-\height-\SidebarFigureYSep;}
          \xdef\SidebarFigureY{\SidebarFigureY\PtUnit}
        };
      \end{tikzpicture}
    }
  }
  \xdef\SidebarContentList{\NewSidebarFigureList}
}

\fancyhead[LO]{\mySidebar{LO}{fancy}}
\fancyhead[RE]{\mySidebar{RE}{fancy}}

\fancypagestyle{plain}{
  \fancyhead[LO]{\mySidebar{LO}{plain}}
  \fancyhead[RE]{\mySidebar{RE}{plain}}
}

\let\cleardoublepage=\clearpage
\usepackage{etoolbox}
\makeatletter
\patchcmd{\chapter}{\if@openright\cleardoublepage\else\clearpage\fi}{}{}{}
\makeatother

% Sidebar figure list

\xdef\SidebarContentList{}
\xdef\SidebarFigureCounter{1}
\xdef\SidebarFigureVPadding{1cm}
\xdef\SidebarFigureYSep{1cm}
\tikzmath{
  \SidebarFigureYEnd=-\paperheight+\botSep+\SidebarFigureVPadding;
}
\xdef\SidebarFigureYEnd{\SidebarFigureYEnd\PtUnit}
\newlength{\SidebarFigureHeight}

\NewEnviron{sidebarFigure}{
  % Make the box which is the figure content
  \def\SidebarContentName{SidebarFigure\SidebarFigureCounter}
  \edef\CommandFigureName{\csname \SidebarContentName\endcsname}
  \expandafter\newsavebox\CommandFigureName
  \begin{lrbox}{\CommandFigureName}
    \calcWidth{1}%
    \begin{minipage}{\customFigureWidth}%
      \vspace{-\floatsep}%
      \begin{figure}[H]
        \centering
        \BODY%
      \end{figure}
    \end{minipage}%
  \end{lrbox}
  % \begin{lrbox}{\CommandFigureName}\BODY\end{lrbox}
  \global%
  \expandafter\setbox\CommandFigureName%
  \expandafter\box\CommandFigureName
  % Add to list
  \AddToList{\SidebarContentList}{\SidebarContentName}
  % Update counter
  \tikzmath{\SidebarFigureCounter=int(\SidebarFigureCounter+1);}
  \xdef\SidebarFigureCounter{\SidebarFigureCounter}
}

\newcounter{Comment}
\setcounter{Comment}{0}

\makeatletter
\define@key{sidebarCommentKeys}{clabel}{\def\clabel{#1}}%
\define@key{sidebarCommentKeys}{yshift}{\def\yshift{#1}}%
\makeatother
\newcommand{\sidebarComment}[2][]{%
  \setkeys{sidebarCommentKeys}{clabel=,#1}%
  \refstepcounter{Comment}%
  \ifthenelse{\equal{\clabel}{}}{}{\label{footnote:\clabel}}%
  $^{\textnormal{\ref{footnote:\theComment}}}$%
  % Make the box which is the comment content
  \def\SidebarContentName{SidebarFigure\SidebarFigureCounter}%
  \edef\CommandFigureName{\csname \SidebarContentName\endcsname}%
  \expandafter\newsavebox\CommandFigureName%
  \begin{lrbox}{\CommandFigureName}%
    \calcWidth{1}%
    \begin{minipage}{\customFigureWidth}%
      \protect\label{footnote:\theComment}$^{\theComment}$ #2%
    \end{minipage}%
  \end{lrbox}%
  \global%
  \expandafter\setbox\CommandFigureName%
  \expandafter\box\CommandFigureName%
  % Add to list
  \AddToList{\SidebarContentList}{\SidebarContentName}%
  % Update counter
  \tikzmath{\SidebarFigureCounter=int(\SidebarFigureCounter+1);}%
  \xdef\SidebarFigureCounter{\SidebarFigureCounter}%
}

\newcommand{\AddToList}[2]{%
  % #1: list variable
  % #2: element
  \ifthenelse{\equal{#1}{}}{\xdef#1{#2}}{\xdef#1{#1,#2}}%
}

% Math theorem envs
\def\thmVSpace{3mm}%

\newcommand{\bookProof}[1][]{\vspace{\thmVSpace}\noindent{\itshape Proof%
    \ifthenelse{\equal{#1}{}}{}{~(#1)}.}\hspace{4mm}}

\makeatletter
\define@key{theoremKeys}{type}{\def\type{#1}}%
\define@key{theoremKeys}{tlabel}{\def\tlabel{#1}}%
\makeatother

\newcounter{Booktheorem}
\newcounter{Bookdefinition}
\newcounter{Bookcorollary}
\newcounter{Booklemma}
\newcounter{Bookproposition}
\newcounter{Bookcondition}
\newcounter{Bookassumption}
\newcounter{Bookexample}
\newcounter{BookThmCounter}
\setcounter{Booktheorem}{0}
\setcounter{Bookdefinition}{0}
\setcounter{Bookcorollary}{0}
\setcounter{Booklemma}{0}
\setcounter{Bookproposition}{0}
\setcounter{Bookcondition}{0}
\setcounter{Bookassumption}{0}
\setcounter{Bookexample}{0}
\setcounter{BookThmCounter}{1}

\newcounter{qedCounter}
\setcounter{qedCounter}{1}
\renewcommand{\qedsymbol}{}
\newcommand{\qedmark}{%
  \pgfmark{qedmark\theqedCounter}%
  \stepcounter{qedCounter}%
}

\NewEnviron{bookTheorem}[1][]{%
  % Parameters%
  \setkeys{theoremKeys}{type=theorem,#1}%
  \setkeys{theoremKeys}{tlabel=,#1}%
  % HEADING
  \ifthenelse{\equal{\type}{}}{}{%
    \edef\CounterName{Book\type}%
    \refstepcounter{\CounterName}%
    \edef\name{\capitalisewords{\type}~\arabic{\CounterName}}%
    \label{\type:\tlabel}%
    % Title
    \vspace{\thmVSpace}%
    \edef\markNameStart{defStart\theBookThmCounter}%
    \edef\markNameEnd{defEnd\theBookThmCounter}%
    {\noindent\pgfmark{\markNameStart}\phantom{\bfseries\name.}}\pgfmark{\markNameEnd}
    \begin{tikzpicture}[remember picture,overlay]%
      \tikzmath{
        \pad = 1mm;
        \height = 0.7em+2*\pad;
        \Angle = 60;
        \tipOffset = \height*tan(90-\Angle);
        \tipOffsetValueLocal = 2.5*\tipOffset;
      }
      \xdef\tipOffsetValue{\tipOffsetValueLocal\PtUnit}
      \tikzset{
        theorem background/.append style={
          fill=black!10,
          draw=black!30,
          line width=0.4mm
        }
      }
      \coordinate (south west) at (pic cs:\markNameStart);
      \coordinate (south east) at (pic cs:\markNameEnd);
      \draw[theorem background]
      ($(south west)+(0,-\pad*1pt)$) to
      ($(south east)+(2*\pad*1pt,-\pad*1pt)$) to
      ++({(\tipOffset+\pad)*1pt},\height*1pt) to
      ($(south west)+(0,-\pad*1pt)+(0,\height*1pt)$) to
      cycle;
      \node[anchor=north west,inner sep=0,outer sep=0,font={\bfseries}] at ($(south west)+(\pad*1pt,\height*1pt-2*\pad*1pt)$) {\name.};
    \end{tikzpicture}%
    \hspace{\tipOffsetValue}%
  }%
  % BODY
  \BODY\ifthenelse{\equal{\theqedCounter}{\theBookThmCounter}}{\qedmark}{}%
  \stepcounter{BookThmCounter}%
  \addtocounter{qedCounter}{-1}%
  % QED
  \begin{tikzpicture}[remember picture,overlay]%
    \def\qedSz{0.7em}
    \tikzset{
      QED/.style={
        anchor=south west,
        rectangle,
        inner sep=0,
        outer sep=0,
        minimum size=\qedSz,
        fill=white,
        draw=black
      }
    }
    \path let
    \p1=(pic cs:qedmark\theqedCounter),
    \p2=(current page.east)
    in \pgfextra{
      \ifthispageodd{
        \tikzmath{\xloc=\x2-\outerSep+\qedSz;}
      }{
        \tikzmath{\xloc=\x2-\innerSep+\qedSz;}
      }
      \node[QED] at (\xloc*1pt,\y1) {};
    };
  \end{tikzpicture}%
  \addtocounter{qedCounter}{1}%
  \vspace{\thmVSpace}%
}

% List style
\def\EnumMargin{2cm}
\NewEnviron{bookList}{
  \begin{enumerate}[
    leftmargin=\textMarginWidthUnits,
    rightmargin=\textMarginWidthUnits,
    align=left,
    labelwidth=0.7em,
    labelsep=0pt,
    label=\protect\fancyarrow
    ]
    \BODY
  \end{enumerate}
}

% Bibliography style
\setlength{\bibsep}{1pt}
\def\bibfont{\footnotesize}
\gappto{\UrlBreaks}{\UrlOrds}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/csm_style.tex <==
% ..:: Compilattion mode ::..

\ifthenelse{\isundefined{\preprintcsm}}{
  \makeflag{prettycsm}{true}}{
  \makeflag{prettycsm}{false}}

% ..:: Preamble ::..

\ifmakeprettycsm
\else
\usepackage{csm16}
\usepackage[margin=1in]{geometry}
\usepackage[nolists,nomarkers,tablesfirst]{endfloat} % put figures at end

% added for CSMAG only
\usepackage{url}
\usepackage{graphicx,xcolor}
\usepackage{verbatim}% http://ctan.org/pkg/verbatim
\makeatletter
\newcommand{\verbatimfont}[1]{\def\verbatim@font{#1}}%
\makeatother
\verbatimfont{\ttfamily\small}
\newcommand{\XX}[1]{{\bf XX #1 XX}}
\newcommand{\bi}{\begin{itemize}}\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{equation}}\newcommand{\ee}{\end{equation}}
\newcommand{\bee}{\begin{enumerate}}\newcommand{\eee}{\end{enumerate}}
\newcommand{\bea}{\begin{eqnarray}}\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beas}{\begin{eqnarray*}}\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bc}{\begin{center}}\newcommand{\ec}{\end{center}}
%
\usepackage[left,pagewise]{lineno}
\usepackage[english]{babel}
\usepackage{blindtext}
% added for CSMAG only

\newif\ifPDF \ifx\pdfoutput\undefined\PDFfalse \else \ifnum\pdfoutput > 0\PDFtrue \else\PDFfalse \fi
\ifPDF
\usepackage[pdftex, plainpages = false, colorlinks=true, linkcolor=black, citecolor = green!50!blue, urlcolor = blue, filecolor=black, pagebackref=false, hypertexnames=false,  pdfpagelabels ]{hyperref}
\fi

\gdef\csmpreprintfigscale{1.1}

\fi

% ..:: Colors ::..

\makeatletter

\definecolor{csm@intro@first@char}{HTML}{df9434}
\definecolor{csm@sidebar@bg}{HTML}{f2e9c4}
\definecolor{csm@sidebar@first@char}{HTML}{a08c2f}
\definecolor{csm@fig@bg}{HTML}{e6f7fe}
\definecolor{@light@blue}{HTML}{26baf2}
\colorlet{csm@fig@label@body}{@light@blue}
\colorlet{csm@blurb@color}{@light@blue}
\definecolor{@golden}{HTML}{c8b03b}
\colorlet{csm@fig@label@sidebar}{@golden}
\colorlet{csm@abstract@color}{@golden}
\definecolor{csm@table@caption@bg}{HTML}{abc2e9}
\definecolor{csm@table@border}{HTML}{5e81c9}
\colorlet{csm@table@bg}{csm@fig@bg}

\makeatother

% ..:: Paragraphs ::..

\ifmakeprettycsm
\makeatletter
\def\@csm@parindent{1em}
\def\@csm@parskip{0pt plus1pt}

\setlength\parindent{\@csm@parindent} % Paragraph indentation
\setlength{\parskip}{\@csm@parskip} % Paragraph spacing

\makeatother
\fi

% ..:: Fonts ::..

\ifmakeprettycsm
% \let\transp\relax
% \usepackage{newtxmath}
\let\temp\rmdefault
\usepackage{mathpazo}
\let\rmdefault\temp

\DeclareMathSizes{10}{9}{7}{5}

% See https://tex.stackexchange.com/a/195867/90535
\DeclareSymbolFont{Greekletters}{OT1}{iwona}{m}{n}
\DeclareSymbolFont{greekletters}{OML}{iwona}{m}{it}
\DeclareMathSymbol{\Delta}{\mathord}{Greekletters}{"01}
\DeclareMathSymbol{\Theta}{\mathord}{Greekletters}{"02}
\DeclareMathSymbol{\Lambda}{\mathord}{Greekletters}{"03}
\DeclareMathSymbol{\Xi}{\mathord}{Greekletters}{"04}
\DeclareMathSymbol{\Pi}{\mathord}{Greekletters}{"05}
\DeclareMathSymbol{\Sigma}{\mathord}{Greekletters}{"06}
\DeclareMathSymbol{\Upsilon}{\mathord}{Greekletters}{"07}
\DeclareMathSymbol{\Phi}{\mathord}{Greekletters}{"08}
\DeclareMathSymbol{\Psi}{\mathord}{Greekletters}{"09}
\DeclareMathSymbol{\Omega}{\mathord}{Greekletters}{"0A}
\DeclareMathSymbol{\alpha}{\mathord}{greekletters}{"0B}
\DeclareMathSymbol{\beta}{\mathord}{greekletters}{"0C}
\DeclareMathSymbol{\gamma}{\mathord}{greekletters}{"0D}
\DeclareMathSymbol{\delta}{\mathord}{greekletters}{"0E}
\DeclareMathSymbol{\epsilon}{\mathord}{greekletters}{"0F}
\DeclareMathSymbol{\zeta}{\mathord}{greekletters}{"10}
\DeclareMathSymbol{\eta}{\mathord}{greekletters}{"11}
\DeclareMathSymbol{\theta}{\mathord}{greekletters}{"12}
\DeclareMathSymbol{\iota}{\mathord}{greekletters}{"13}
\DeclareMathSymbol{\kappa}{\mathord}{greekletters}{"14}
\DeclareMathSymbol{\lambda}{\mathord}{greekletters}{"15}
\DeclareMathSymbol{\mu}{\mathord}{greekletters}{"16}
\DeclareMathSymbol{\nu}{\mathord}{greekletters}{"17}
\DeclareMathSymbol{\xi}{\mathord}{greekletters}{"18}
\DeclareMathSymbol{\pi}{\mathord}{greekletters}{"19}
\DeclareMathSymbol{\rho}{\mathord}{greekletters}{"1A}
\DeclareMathSymbol{\sigma}{\mathord}{greekletters}{"1B}
\DeclareMathSymbol{\tau}{\mathord}{greekletters}{"1C}
\DeclareMathSymbol{\upsilon}{\mathord}{greekletters}{"1D}
\DeclareMathSymbol{\phi}{\mathord}{greekletters}{"1E}
\DeclareMathSymbol{\chi}{\mathord}{greekletters}{"1F}
\DeclareMathSymbol{\psi}{\mathord}{greekletters}{"20}
\DeclareMathSymbol{\omega}{\mathord}{greekletters}{"21}
\DeclareMathSymbol{\varepsilon}{\mathord}{greekletters}{"22}
\DeclareMathSymbol{\vartheta}{\mathord}{greekletters}{"23}
\DeclareMathSymbol{\varpi}{\mathord}{greekletters}{"24}
\DeclareMathSymbol{\varrho}{\mathord}{greekletters}{"25}
\DeclareMathSymbol{\varsigma}{\mathord}{greekletters}{"26}
\DeclareMathSymbol{\varphi}{\mathord}{greekletters}{"27}

% Fix the prime symbol
\let\oldprime\prime
\renewcommand{\prime}{^\oldprime}
\newcommand{\pprime}{''}
\newcommand{\ppprime}{'''}
% \newcommand\der{\mkern+0mu\raise-0.0ex\hbox{$\scriptstyle\prime$}}
\newcommand\der{^{\mkern+2.5mu\raise-3pt\hbox{$\scriptstyle\prime$}}}
\else
\newcommand\der{'}
\fi
\newcommand\dder{\der\der}
\newcommand\ddder{\der\der\der}
\newcommand\dddder{\der\der\der\der}

% ..:: Lists ::..

\ifmakeprettycsm
\tikzset{
  list bullet/.style={
    scale=0.5
  }
}

\setlist[itemize,1]{label={%
    \tikz[outer sep=0,inner sep=0,baseline=-0.3em]{%
      \node[list bullet] at (0,0) {\faChevronRight};%
      \node[list bullet] at (0.25em,0) {\faChevronRight};}%
  },leftmargin=1.3em}
\fi

% ..:: Page geometry ::..

\ifmakeprettycsm
\usepackage{geometry}

\ExplSyntaxOn
\tl_set:Nn \l_sidemargin_dim {1.5cm}
\tl_set:Nn \l_topmargin_dim {2.2cm}
\tl_set:Nn \l_botmargin_dim {1.6cm}
\tl_set:Nn \l_footmargin_dim {6mm}
\tl_set:Nn \l_columnsep_dim {3mm}
\geometry{
  papersize={200mm,273mm},
  twocolumn,
  left=\tl_use:N \l_sidemargin_dim,
  right=\tl_use:N \l_sidemargin_dim,
  top=\tl_use:N \l_topmargin_dim,
  bottom=\tl_use:N \l_botmargin_dim,
  footskip=\tl_use:N \l_footmargin_dim,
  columnsep=\tl_use:N \l_columnsep_dim
}
\ExplSyntaxOff
\fi

% ..:: Section titles ::..

\ifmakeprettycsm
\usepackage{helvet}
\titleformat{\section}{%
  \normalfont\fontsize{10}{12}%
  \sffamily\bfseries\MakeUppercase}{}{0cm}{#1}
\titlespacing*{\section}{0cm}{4mm}{0mm}

\titleformat{\subsection}{%
  \normalfont\fontsize{10}{12}%
  \sffamily\bfseries\slshape}{}{0cm}{#1}
\titlespacing*{\subsection}{0cm}{4mm}{0mm}

\titleformat{\subsubsection}{%
  \normalfont\fontsize{10}{12}%
  \sffamily}{}{0cm}{#1}
\titlespacing*{\subsubsection}{0cm}{4mm}{0mm}
\fi

% >> Opening text <<

\makeatletter

\ifmakeprettycsm
\newcommand{\firstword}[2][]{%
  \StrChar{#2}{1}[\first@char]%
  \StrBehind{#2}{\first@char}[\rest@of@word]%
  \renewcommand{\LettrineFontHook}{\sffamily\bfseries}%
  \lettrine[lines=5,#1]{%
    \color{csm@intro@first@char}%
    \first@char}{\rest@of@word}%
}
\else
\newcommand{\firstword}[2][]{#2}
\fi

\makeatother

% ..:: Header and footer ::..

\ifmakeprettycsm
\usepackage{fontawesome}

\ExplSyntaxOn
\tl_new:N \l_csm_date
\tl_set:Nn \l_csm_date {}

\newcommand{\csmdate}[1]{
  \tl_set:Nn \l_csm_date {#1}
}

\fancypagestyle{csmfancy}{%
  \fancyhf{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyfoot[LO]{%
    \sffamily%
    \fontsize{9}{11}%
    \textbf{\thepage}~~%
    \fontsize{6}{8}%
    \textbf{IEEE~CONTROL~SYSTEMS}~~%
    \tikz[outer~sep=0,inner~sep=0]{%
      \node[scale=0.8] at (0,0) {\faChevronRight};%
      \node[scale=0.8] at (0.4em,0) {\faChevronRight};}%
    {\normalfont\sffamily{}~\tl_use:N \l_csm_date}%
  }%
  \fancyfoot[RE]{%
    \fontsize{6}{8}%
    \sffamily%
    {\tl_use:N \l_csm_date}~%
    \tikz[outer~sep=0,inner~sep=0]{%
      \node[scale=0.8] at (0,0) {\faChevronLeft};%
      \node[scale=0.8] at (0.4em,0) {\faChevronLeft};}%
    \textbf{~IEEE~CONTROL~SYSTEMS}%
    \fontsize{9}{11}%
    \textbf{~~\thepage}%
  }%
}
\pagestyle{csmfancy}
\ExplSyntaxOff
\else
\newcommand{\csmdate}[1]{}
\fi

% ..:: Equations ::..

\allowdisplaybreaks

% ..:: Theorem environments ::..

\ifmakeprettycsm
\makeatletter

% >> Set the theorem environment style <<

\newtheoremstyle{csm@theorem@style}% name
{4mm}% Space above
{1pt}% Space below
{}% Body font
{}% Indent amount
{\fontsize{9}{11}\sffamily}% Theorem head font
{}% Punctuation after theorem head
{\newline}% Space after theorem head
{}% Theorem head spec(can be left empty, meaning ‘normal’)

\theoremstyle{csm@theorem@style}

% >> Define the "basic" theorem environments <<

\newtheorem{csm@theorem}{Theorem}
\newtheorem{csm@lemma}{Lemma}
\newtheorem{csm@corollary}{Corollary}
\newtheorem{csm@proposition}{Proposition}
\newtheorem{csm@remark}{Remark}
\newtheorem{csm@property}{Property}
\newtheorem{csm@condition}{Condition}
\newtheorem{csm@method}{Method}
\newtheorem{csm@example}{Example}
\newtheorem{csm@problem}{Problem}
\newtheorem{csm@definition}{Definition}
\newtheorem{csm@assumption}{Assumption}

% >> Update basic theorem environments with extra elements <<

\def\@thmenvs{theorem,lemma,corollary,proposition,remark,property,%
  condition,method,example,problem,definition,assumption}

\foreach \@te in \@thmenvs {
  \bgroup
  \globaldefs=1
  % Save the original definition
  \expandafter\let\csname ocsm@\@te\expandafter\endcsname
  \csname csm@\@te\endcsname
  \expandafter\let\csname eocsm@\@te\expandafter\endcsname
  \csname endcsm@\@te\endcsname
  % Re-define the environment
  \renewenvironment{\@te}[1][]{%
    \csname ocsm@\@currenvir\endcsname%
    \ifthenelse{\equal{##1}{}}{}{\label{\@currenvir:##1}}
  }{%
    \hfill$\blacksquare$% % "QED"
    \expandafter\csname eocsm@\@currenvir\endcsname%
  }
  \egroup
}

\makeatother
\fi

% ..:: Figures ::..

\ExplSyntaxOn
\makeatletter

\tl_new:N \l_csm_figure_label_tl
\tl_new:N \l_csm_figure_caption_tl
\tl_new:N \l_csm_figure_pos_tl
\tl_new:N \l_csm_figure_cols_tl

\define@key{csm@figure@keys}{label}{\tl_set:Nn \l_csm_figure_label_tl {#1}}
\define@key{csm@figure@keys}{caption}{\tl_set:Nn \l_csm_figure_caption_tl {#1}}
\define@key{csm@figure@keys}{position}{\tl_set:Nn \l_csm_figure_pos_tl {#1}}
\define@key{csm@figure@keys}{columns}{\tl_set:Nn \l_csm_figure_cols_tl {#1}}

\ifmakeprettycsm
\newtcolorbox{figurebox}{
  % Drawing engine
  enhanced~jigsaw,
  % Sizes
  width=\linewidth,
  arc=2mm,
  boxrule=0pt,
  titlerule=0pt,
  left=3mm,
  right=3mm,
  bottom=3mm,
  top=3mm,
  boxsep=\tcb@boxsep,
  % Colors
  colback=csm@fig@bg,
  colbacktitle=csm@fig@bg
}

% Caption style
\captionsetup[figure]{font={footnotesize,sf},labelfont={},
  name={\bfseries\color{csm@fig@label@body}FIGURE~},labelsep=space}

% Figure selector
\newenvironment{figure@internal}[2][tbp]{%
  \def\fig@width{#2}%
  \ifthenelse{\equal{\fig@width}{}}{%
    \begin{figure}[#1]}{\begin{figure*}[#1]}}{%
      \ifthenelse{\equal{\fig@width}{}}{%
      \end{figure}}{\end{figure*}}}

\newenvironment{csmfigure}[1][]{%
  % Options
  \setkeys{csm@figure@keys}{label=,#1}%
  \setkeys{csm@figure@keys}{caption=,#1}%
  \setkeys{csm@figure@keys}{position=tbp,#1}%
  \setkeys{csm@figure@keys}{columns=1,#1}%
  % Parse options
  \edef\csm@fig@pos{\tl_use:N \l_csm_figure_pos_tl}%
  \pgfmathparse{\tl_use:N \l_csm_figure_cols_tl ==1 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    \gdef\csm@figure@width{}%
  }{%
    \gdef\csm@figure@width{dbl}%
  }%
  % Make igure
  \edef\begin@figure@cmd{{figure@internal}[\csm@fig@pos}%
  \expandafter\begin\begin@figure@cmd]{\csm@figure@width}%
    \begin{figurebox}
    }{%
    \end{figurebox}
    \caption{\tl_use:N \l_csm_figure_caption_tl}
    \figlabel{\tl_use:N \l_csm_figure_label_tl}
  \end{figure@internal}
}
\else
\gdef\csm@singlecol@emulate@width{0.7}
\newenvironment{csmfigure}[1][]{%
  % Options
  \setkeys{csm@figure@keys}{label=,#1}%
  \setkeys{csm@figure@keys}{caption=,#1}%
  \setkeys{csm@figure@keys}{position=tbp,#1}%
  \setkeys{csm@figure@keys}{columns=1,#1}%
  % Parse options
  \edef\csm@num@cols{\tl_use:N \l_csm_figure_cols_tl}
  \pgfmathparse{\csm@num@cols>1 ? 1:0}
  \ifthenelse{\pgfmathresult>0}{\def\csm@figarea@width{1}}{%
    \def\csm@figarea@width{\csm@singlecol@emulate@width}}
  % Make figure
  \begin{figure}
    \centering
    \begin{minipage}{\csm@figarea@width\textwidth}
    }{%
    \end{minipage}
    \caption{\tl_use:N \l_csm_figure_caption_tl}
    \figlabel{\tl_use:N \l_csm_figure_label_tl}
  \end{figure}
}
\DeclareDelayedFloatFlavor{csmfigure}{figure}
\fi

\makeatother
\ExplSyntaxOff

% Reference a subfigure that is baked into the drawing, so not really a LaTeX
% subfigure
\newcommand{\fakesubfigref}[3][]{%
  \figref{#2}(#3)\ifthenelse{\equal{#1}{}}{}{-(#1)}}

% ..:: Tables ::..

\ExplSyntaxOn
\makeatletter

\tl_new:N \l_csm_table_label_tl
\tl_new:N \l_csm_table_caption_tl
\tl_new:N \l_csm_table_pos_tl
\tl_new:N \l_csm_table_cols_tl

\define@key{csm@table@keys}{label}{\tl_set:Nn \l_csm_table_label_tl {#1}}
\define@key{csm@table@keys}{caption}{\tl_set:Nn \l_csm_table_caption_tl {#1}}
\define@key{csm@table@keys}{position}{\tl_set:Nn \l_csm_table_pos_tl {#1}}
\define@key{csm@table@keys}{columns}{\tl_set:Nn \l_csm_table_cols_tl {#1}}

\ifmakeprettycsm
\def\@table@inner@pad{3mm}
\def\@table@border@width{1pt}

\newtcolorbox{tablebox}[1][]{
  % Drawing engine
  enhanced~jigsaw,
  % Fonts
  fonttitle=\sffamily\bfseries\small,
  fontupper=\sffamily,
  % Sizes
  width=\linewidth,
  arc=2mm,
  boxrule=\@table@border@width,
  titlerule=\@table@border@width,
  left=\@table@inner@pad,
  right=\@table@inner@pad,
  bottom=\@table@inner@pad,
  top=\@table@inner@pad,
  toptitle=\@table@inner@pad,
  bottomtitle=\@table@inner@pad,
  boxsep=\tcb@boxsep,
  % Colors
  colback=csm@table@bg,
  coltitle=black,
  colbacktitle=csm@table@caption@bg,
  colframe=csm@table@border,
  % Title
  title={#1},
  attach~boxed~title~to~top,
  boxed~title~style={colframe=csm@table@border,rounded~corners}
}

% Figure selector
\newenvironment{table@internal}[2][tbp]{%
  \def\table@width{#2}%
  \ifthenelse{\equal{\table@width}{}}{%
    \begin{table}[#1]}{\begin{table*}[#1]}}{%
      \ifthenelse{\equal{\table@width}{}}{%
      \end{table}}{\end{table*}}}

\newenvironment{csmtable}[1][]{%
  % Options
  \setkeys{csm@table@keys}{label=,#1}%
  \setkeys{csm@table@keys}{caption=,#1}%
  \setkeys{csm@table@keys}{position=tbp,#1}%
  \setkeys{csm@table@keys}{columns=1,#1}%
  % Parse options
  \edef\csm@table@pos{\tl_use:N \l_csm_table_pos_tl}%
  \pgfmathparse{\tl_use:N \l_csm_table_cols_tl ==1 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    \gdef\csm@table@width{}%
  }{%
    \gdef\csm@table@width{dbl}%
  }%
  % Make figure
  \edef\begin@table@cmd{{table@internal}[\csm@table@pos}%
    \expandafter\begin\begin@table@cmd]{\csm@table@width}%
    \refstepcounter{table}
    \begin{tablebox}[%
      {\bfseries TABLE~\arabic{table}}\hspace{1em}%
      \tl_use:N \l_csm_table_caption_tl]%
      \fontsize{9}{13}%
    }{%
    \end{tablebox}
    \tablabel{\tl_use:N \l_csm_table_label_tl}
  \end{table@internal}
}
\else
\newenvironment{csmtable}[1][]{%
  % Options
  \setkeys{csm@table@keys}{label=,#1}%
  \setkeys{csm@table@keys}{caption=,#1}%
  \setkeys{csm@table@keys}{position=tbp,#1}%
  \setkeys{csm@table@keys}{columns=1,#1}%
  % % Parse options
  \edef\csm@num@cols{\tl_use:N \l_csm_table_cols_tl}
  \pgfmathparse{\csm@num@cols>1 ? 1:0}
  \ifthenelse{\pgfmathresult>0}{\def\csm@tabarea@width{1}}{%
    \def\csm@tabarea@width{\csm@singlecol@emulate@width}}
  % Make figure
  \begin{table}[t]
    \caption{\tl_use:N \l_csm_table_caption_tl}
    \vspace*{.1in}
    \centering
    \begin{minipage}{\csm@tabarea@width\textwidth}
    }{%
    \end{minipage}
    \tablabel{\tl_use:N \l_csm_table_label_tl}
  \end{table}
}
\DeclareDelayedFloatFlavor{csmtable}{table}
\fi

\makeatother
\ExplSyntaxOff

% ..:: Referencing ::..

\makeatletter

% Source: https://tex.stackexchange.com/a/168835/90535
\let\oldhypertarget\hypertarget
\renewcommand{\hypertarget}[2]{%
  \oldhypertarget{#1}{#2}%
  \protected@write\@mainaux{}{%
    \string\expandafter\string\gdef
    \string\csname\string\detokenize{#1}\string\endcsname{#2}%
  }%
}

\newcommand{\csmhyperlink}[1]{%
  \hyperlink{#1}{\csname #1\endcsname}%
}

\makeatother

% ..:: Sidebars ::..

\ExplSyntaxOn
\makeatletter

\tl_new:N \l_csm_sidebar_title_tl
\tl_new:N \l_csm_sidebar_label_tl
\tl_new:N \l_csm_sidebar_side_tl
\tl_new:N \l_csm_sidebar_pos_tl
\tl_new:N \l_csm_sidebar_cols_tl

\define@key{csm@sidebar@keys}{title}{\tl_set:Nn \l_csm_sidebar_title_tl {#1}}
\define@key{csm@sidebar@keys}{label}{\tl_set:Nn \l_csm_sidebar_label_tl {#1}}
\define@key{csm@sidebar@keys}{side}{\tl_set:Nn \l_csm_sidebar_side_tl {#1}}
\define@key{csm@sidebar@keys}{position}{\tl_set:Nn \l_csm_sidebar_pos_tl {#1}}
\define@key{csm@sidebar@keys}{columns}{\tl_set:Nn \l_csm_sidebar_cols_tl {#1}}

\newcounter{sidebar@equation}%
\newcounter{sidebar@table}%
\newcounter{sidebar@figure}%
\newcounter{subsidebar@counter}

\setcounter{subsidebar@counter}{0}

% Keep track of how many references the sidebar bibliography has
\newcounter{sbrefs}
\renewbibmacro*{finentry}{\stepcounter{sbrefs}\finentry}

% Low-level print sidebar bibliography
\newcommand{\csm@sb@printbib}[2]{%
  \printbibliography[title=References,keyword=#1,resetnumbers=#2]}

% Print a sidebar bibliography with new references specifically for the sidebar
\newcommand{\make@sidebar@bib}{%
  \edef\sidebar@bib@label{sidebar:\tl_use:N \l_csm_sidebar_label_tl}%
  % Decision whether to reset the reference counter
  \ifmakeprettycsm
  \def\@sb@bibnum@reset{false}%
  \else
  \pgfmathparse{\thesbrefs==0 ? 1:0}
  % \ifthenelse{\equal{\@sidebar@number}{1}}{%
  \ifthenelse{\pgfmathresult>0}{%
    \def\@sb@bibnum@reset{true}
  }{%
    \def\@sb@bibnum@reset{false}
  }%
  \fi
  % Print the bibliography, citations start with an "S"
  \begin{refcontext}[sorting=none,labelprefix=S]%
    \ifmakeprettycsm
    \renewcommand*{\bibfont}{\fontsize{7}{9}\sffamily}%
    \else
    \renewcommand*{\bibfont}{\footnotesize}%
    \fi
    \DeclareFieldFormat{labelnumberwidth}{[##1]}%
    \begingroup\edef\sidebar@print@bib{\endgroup\noexpand
      \printbibliography[title=References,
      keyword=\sidebar@bib@label,
      resetnumbers=\@sb@bibnum@reset]
    }\sidebar@print@bib
  \end{refcontext}%
}

% Prefix labels with "S" for sidebar
\newcommand{\sidebar@labels@on}{
  \global\chardef\dc@currentequation=\value{equation}%
  \global\chardef\dc@currentfigure=\value{figure}%
  \global\chardef\dc@currenttable=\value{table}%
  \let\c@equation\c@sidebar@equation
  \let\c@figure\c@sidebar@figure
  \let\c@table\c@sidebar@table
  \renewcommand{\theequation}{S\arabic{equation}}%
  \renewcommand{\thetable}{S\arabic{table}}%
  \renewcommand{\thefigure}{S\arabic{figure}}%
  \renewcommand{\theHequation}{S\arabic{equation}}%
  \renewcommand{\theHtable}{S\arabic{table}}%
  \renewcommand{\theHfigure}{S\arabic{figure}}%
}

% Reset labels to original
\newcommand{\sidebar@labels@off}{
  \edef\equation@mem{\arabic{sidebar@equation}}%
  \edef\figure@mem{\arabic{sidebar@figure}}%
  \edef\table@mem{\arabic{sidebar@table}}%
  \setcounter{equation}{\dc@currentequation}%
  \setcounter{figure}{\dc@currentfigure}%
  \setcounter{table}{\dc@currenttable}%
  \setcounter{sidebar@equation}{\equation@mem}%
  \setcounter{sidebar@figure}{\figure@mem}%
  \setcounter{sidebar@table}{\table@mem}%
}

\ifmakeprettycsm

\newsavebox{\sidebar@box@full}
\newsavebox{\sidebar@box@left}
\newsavebox{\sidebar@box@right}

\def\tcb@left{1em}
\def\tcb@right{1em}
\def\tcb@bottom{1em}
\def\tcb@boxsep{0pt}
\def\tcb@leftfill{0cm}
\def\tcb@rightfill{0cm}

\def\continued@message{\textit{(continued...)}}

\newtcolorbox{sidebarbox}[1][]{
  % Drawing engine
  enhanced~jigsaw,
  % Fonts
  fonttitle=\sffamily\bfseries\large,
  % Sizes
  width=#1,
  arc=2mm,
  boxrule=0pt,
  titlerule=0pt,
  toptitle=2mm,
  left=\tcb@left,
  right=\tcb@right,
  bottom=\tcb@bottom,
  boxsep=\tcb@boxsep,
  leftrule=\tcb@leftfill,
  grow~to~left~by=\tcb@leftfill,
  rightrule=\tcb@rightfill,
  grow~to~right~by=\tcb@rightfill,
  % Colors
  colback=csm@sidebar@bg,
  colframe=csm@sidebar@bg,
  colbacktitle=csm@sidebar@bg,
  coltitle=black
}

\newenvironment{sidebar}[1][]{%
  % Raw options
  \setkeys{csm@sidebar@keys}{title=,#1}%
  \setkeys{csm@sidebar@keys}{label=,#1}%
  \setkeys{csm@sidebar@keys}{side=odd,#1}%
  \setkeys{csm@sidebar@keys}{position=t,#1}%
  \setkeys{csm@sidebar@keys}{columns=2,#1}%
  % Parse options
  \edef\sidebar@side{\tl_use:N \l_csm_sidebar_side_tl}%
  \edef\fig@pos{\tl_use:N \l_csm_sidebar_pos_tl}%
  \pgfmathparse{\tl_use:N \l_csm_sidebar_cols_tl ==1 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    \gdef\figure@width{}%
    \tikzmath{\sidebar@box@width=\columnwidth;
      \sidebar@width=\sidebar@box@width-\tcb@left-\tcb@right-\tcb@boxsep;}
    \xdef\sidebar@box@width{\sidebar@box@width pt}%
    \xdef\sidebar@width{\sidebar@width pt}%
  }{%
    \gdef\figure@width{dbl}%
    \tikzmath{\sidebar@box@width=\textwidth;
      \sidebar@width=\sidebar@box@width-\tcb@left-\tcb@right-\tcb@boxsep;}
    \xdef\sidebar@box@width{\sidebar@box@width pt}%
    \xdef\sidebar@width{\sidebar@width pt}%
  }%
  % Create the box
  \begin{subsidebar}[reset]%
  }{%
  \end{subsidebar}%
  % Draw sidebar
  \pgfmathparse{\value{subsidebar@counter}==1 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    % Show full content in one sidebar
    \sidebar@draw{none}{\sidebar@box@full}%
  }{%
    % Show left and right content in separate sidebars
    \ifthenelse{\equal{\sidebar@side}{odd}}{%
      \def\sidebar@side@other{even}%
    }{%
      \def\sidebar@side@other{odd}%
    }%
    \sidebar@draw{\sidebar@side}{\sidebar@box@left}%
    \sidebar@draw[notitle]{\sidebar@side@other}{\sidebar@box@right}%
  }%
  % Reset counter
  \setcounter{subsidebar@counter}{0}
}

\newcommand{\sidebar@draw}[3][title]{
  \xdef\sidebar@title{\tl_use:N \l_csm_sidebar_title_tl}%
  \xdef\sidebar@label{sidebar:\tl_use:N \l_csm_sidebar_label_tl}%
  \edef\begin@sidebar@cmd{{figure@internal}[\fig@pos}%
  \expandafter\begin\begin@sidebar@cmd]{\figure@width}%
    \ifthenelse{\equal{#1}{title}}{%
      \tcbset{%
        title={\hypertarget{\sidebar@label}{\sidebar@title}}
      }%
    }{}%
    \ifthenelse{\equal{#2}{none}}{%
      \def\tcb@leftfill{0cm}%
      \def\tcb@rightfill{0cm}%
    }{%
      \ifthenelse{\equal{#2}{odd}}{%
        \def\tcb@leftfill{0cm}%
        \def\tcb@rightfill{10cm}%
      }{%
        \def\tcb@leftfill{10cm}%
        \def\tcb@rightfill{0cm}%
      }%
    }%
    \begin{sidebarbox}[\sidebar@box@width]%
      \usebox{#3}%
    \end{sidebarbox}%
  \end{figure@internal}%
}

\newenvironment{subsidebar}[1][noreset]{
  % Options
  \def\sidebar@reset{#1}
  % Check if too many subsidebars
  \pgfmathparse{\value{subsidebar@counter}>=3 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    \PackageError{CSM~style}{Only~two~subsidebars~are~allowed}{}%
  }{}%
  % Get the box name to save content to
  \pgfmathparse{\value{subsidebar@counter}==0 ? 1:0}%
  \ifthenelse{\pgfmathresult>0}{%
    \def\sidebar@box{sidebar@box@full}%
  }{%
    \pgfmathparse{\value{subsidebar@counter}==1 ? 1:0}%
    \ifthenelse{\pgfmathresult>0}{%
      \def\sidebar@box{sidebar@box@left}%
    }{%
      \def\sidebar@box{sidebar@box@right}%
    }%
  }%
  % Increment the counter
  \stepcounter{subsidebar@counter}%
  % Create the box
  \begin{lrbox}{\csname\sidebar@box\endcsname}%
    \begin{minipage}{\sidebar@width}%
      \ifthenelse{\equal{\sidebar@reset}{noreset}}{}{\sidebar@labels@on}%
      % Set columns
      \ifthenelse{\equal{\figure@width}{}}{}{%
        \begin{multicols}{2}%
        }%
        % Set font
        \fontsize{9}{13}
        \setlength\parindent{\@csm@parindent} % Paragraph indentation
        \setlength{\parskip}{\@csm@parskip} % Paragraph spacing
        % \renewcommand\familydefault\sfdefault
        \sffamily\sansmath
        \captionsetup[figure]{name={%
            \bfseries\color{csm@fig@label@sidebar}FIGURE~}}
        % Print "continued" if this is the second subsidebar panel
        \pgfmathparse{\value{subsidebar@counter}==3 ? 1:0}%
        \ifthenelse{\pgfmathresult>0}{%
          \continued@message%
        }{}%
        % Main text body (given environment body) ...
      }{%
        % ... End of main text body
        \pgfmathparse{\value{subsidebar@counter}!=2 ? 1:0}%
        % Print bibliography
        \ifthenelse{\pgfmathresult>0}{%
          \make@sidebar@bib%
        }{}%
        % Print "continued" if this is the first subsidebar panel
        \ifthenelse{\pgfmathresult>0}{}{%
          \continued@message%
        }%
        % End columns
        \ifthenelse{\equal{\figure@width}{}}{}{%
        \end{multicols}%
      }%
      \ifthenelse{\equal{\sidebar@reset}{noreset}}{}{\sidebar@labels@off}%
    \end{minipage}%
  \end{lrbox}%
  % Save the box for global access
  \global%
  \expandafter\setbox\csname\sidebar@box\endcsname%
  \expandafter\box\csname\sidebar@box\endcsname%
}

\else

\newenvironment{sidebar}[1][]{%
  % Raw options
  \setkeys{csm@sidebar@keys}{title=,#1}%
  \setkeys{csm@sidebar@keys}{label=,#1}%
  \setkeys{csm@sidebar@keys}{side=odd,#1}%
  \setkeys{csm@sidebar@keys}{position=t,#1}%
  \setkeys{csm@sidebar@keys}{columns=2,#1}%
  % Parse options
  \edef\@csm@sb@title{\tl_use:N \l_csm_sidebar_title_tl}
  \edef\@csm@sb@label{sidebar:\tl_use:N \l_csm_sidebar_label_tl}%
  % New page
  \clearpage
  \newpage
  % >> Create the sidebar <<
  % Title
  \section[\@csm@sb@title]{Sidebar:~%
    \hypertarget{\@csm@sb@label}{\@csm@sb@title}}
  \sidebar@labels@on % Turn on "S" prefixes
}{
  \make@sidebar@bib
  % Print out the figures
  \newpage
  \processdelayedfloats % place sidebar endfloats here
  \clearpage
  \sidebar@labels@off % Turn off "S" prefixes
}

\newenvironment{subsidebar}[1][noreset]{}{}

\fi

% Define a queue of sidebars that are to be printed
\newcounter{sidebar@queue@size}%
\newcommand{\reset@sidebar@queue}{
  \gdef\csm@sb@queue@title{}
  \gdef\csm@sb@queue@label{}
  \gdef\csm@sb@queue@side{}
  \gdef\csm@sb@queue@position{}
  \gdef\csm@sb@queue@columns{}
  \gdef\csm@sb@queue@content{}
  \setcounter{sidebar@queue@size}{0}
}
\reset@sidebar@queue

% Push a new sidebar into the queue
\newcommand{\declaresidebar}[2][]{
  % Raw options
  \setkeys{csm@sidebar@keys}{title=,#1}%
  \setkeys{csm@sidebar@keys}{label=,#1}%
  \setkeys{csm@sidebar@keys}{side=odd,#1}%
  \setkeys{csm@sidebar@keys}{position=t,#1}%
  \setkeys{csm@sidebar@keys}{columns=2,#1}%
  % Save to queue
  \add@list@item{\csm@sb@queue@title}{\tl_use:N \l_csm_sidebar_title_tl}
  \add@list@item{\csm@sb@queue@label}{\tl_use:N \l_csm_sidebar_label_tl}
  \add@list@item{\csm@sb@queue@side}{\tl_use:N \l_csm_sidebar_side_tl}
  \add@list@item{\csm@sb@queue@position}{\tl_use:N \l_csm_sidebar_pos_tl}
  \add@list@item{\csm@sb@queue@columns}{\tl_use:N \l_csm_sidebar_cols_tl}
  \add@list@item{\csm@sb@queue@content}{#2}
  \stepcounter{sidebar@queue@size}
  % Print sidebars immediately if pretty CSM
  \ifmakeprettycsm
  \flushsidebars
  \fi
}

% Print out all sidebars, removing them from the queue (FIFO)
\makeflag{printsb}{false}
\newcommand{\flushsidebars}{
  % Decide if there are any sidebars to be printed
  \pgfmathparse{\thesidebar@queue@size>0 ? 1:0}
  \ifthenelse{\pgfmathresult>0}{\makeprintsbtrue}{\makeprintsbfalse}
  \ifmakeprintsb
  % Reset the reference counter
  \setcounter{sbrefs}{0}
  % Make sidebar queues into indexable arrays
  \makelist{csm@sb@titles}{\csm@sb@queue@title}
  \makelist{csm@sb@labels}{\csm@sb@queue@label}
  \makelist{csm@sb@sides}{\csm@sb@queue@side}
  \makelist{csm@sb@positions}{\csm@sb@queue@position}
  \makelist{csm@sb@columns}{\csm@sb@queue@columns}
  \makelist{csm@sb@contents}{\csm@sb@queue@content}
  \foreach \@sidebar@number in {1,...,\thesidebar@queue@size} {
    \begin{sidebar}[%
      title={\list@nth{csm@sb@titles}{\@sidebar@number}},
      label={\list@nth{csm@sb@labels}{\@sidebar@number}},
      side={\list@nth{csm@sb@sides}{\@sidebar@number}},
      position={\list@nth{csm@sb@positions}{\@sidebar@number}},
      columns={\list@nth{csm@sb@columns}{\@sidebar@number}}]
      \input{\list@nth{csm@sb@contents}{\@sidebar@number}}
    \end{sidebar}
  }
  \reset@sidebar@queue % Empty the queue
  \fi
}

\ifmakeprettycsm
\renewcommand*{\LettrineTextFont}{}
\newcommand{\sbfirstword}[1]{%
  \StrChar{#1}{1}[\first@char]%
  \StrBehind{#1}{\first@char}[\rest@of@word]%
  \lettrine[nindent=0pt,slope=0pt,findent=3pt]{%
    \color{csm@sidebar@first@char}\bfseries%
    \first@char}{\rest@of@word}%
}
\else
\newcommand{\sbfirstword}[1]{#1}
\fi

\newcommand{\sbref}[1]{%
  \@ifundefined{sidebar:#1}{%
    ``\textbf{??}''%
  }{%
    ``\csmhyperlink{sidebar:#1}''%
  }%
}

\makeatother
\ExplSyntaxOff

% ..:: Highlight text blurb ::..

\ifmakeprettycsm
\makeatletter

\def\blurb@pad{4mm}

\newtcolorbox{blurbbox}{
  % Drawing engine
  enhanced jigsaw,
  % Fonts
  fontupper=\sffamily\bfseries\large,
  % Sizes
  width=\textwidth,
  arc=2mm,
  boxrule=0.5pt,
  titlerule=0pt,
  toptitle=2mm,
  left=\blurb@pad,
  right=\blurb@pad,
  bottom=\blurb@pad,
  top=\blurb@pad,
  boxsep=0pt,
  % Colors
  opacityback=0,
  colframe=csm@blurb@color,
  coltext=csm@blurb@color
}

\newenvironment{blurb}{
  \begin{figure*}[!t]
    \centering
    \begin{blurbbox}
      \centering
      \setlength{\baselineskip}{1.4em}
    }{
    \end{blurbbox}
  \end{figure*}
}

\makeatother
\else
\NewEnviron{blurb}{}
\fi

% ..:: Abstract (which will not appear in print) ::..

\ifmakeprettycsm
\makeatletter

\def\abstract@pad{2mm}

\newtcolorbox{abstractbox}{
  % Drawing engine
  enhanced jigsaw,
  % Fonts
  fontupper=\sffamily,
  % Sizes
  width=\textwidth,
  arc=2mm,
  boxrule=0.5pt,
  titlerule=0pt,
  toptitle=2mm,
  left=\abstract@pad,
  right=\abstract@pad,
  bottom=\abstract@pad,
  top=\abstract@pad,
  boxsep=0pt,
  % Colors
  opacityback=0,
  colframe=csm@abstract@color,
  coltext=black!70
}

\newenvironment{csmabstract}{
  \begin{figure*}[t]
    \centering
    \begin{abstractbox}%
      \paragraph{\sffamily Abstract (hidden in print).}%
    }{%
    \end{abstractbox}
  \end{figure*}
}

\makeatother
\else
\NewEnviron{csmabstract}{}
\fi

% ..:: Nomenclature ::..

\ExplSyntaxOn
\makeatletter

\tl_new:N \l_csm_nomenclature_title_tl
\tl_new:N \l_csm_nomenclature_label_tl
\tl_new:N \l_csm_nomenclature_first_col_width_tl
\tl_new:N \l_csm_nomenclature_position_tl

\define@key{csm@nomenclature@keys}{title}{\tl_set:Nn
  \l_csm_nomenclature_title_tl {#1}}
\define@key{csm@nomenclature@keys}{label}{\tl_set:Nn
  \l_csm_nomenclature_label_tl {#1}}
\define@key{csm@nomenclature@keys}{width}{\tl_set:Nn
  \l_csm_nomenclature_first_col_width_tl {#1}}
\define@key{csm@nomenclature@keys}{position}{\tl_set:Nn
  \l_csm_nomenclature_position_tl {#1}}

\newcommand{\csmnomenclature}[2][]{
  % Raw arguments
  \setkeys{csm@nomenclature@keys}{title=,#1}%
  \setkeys{csm@nomenclature@keys}{label=,#1}%
  \setkeys{csm@nomenclature@keys}{width=0.2,#1}%
  \setkeys{csm@nomenclature@keys}{position=t,#1}%
  % Parse arguments
  \edef\nomenc@title{\tl_use:N
    \l_csm_nomenclature_title_tl}%
  \edef\nomenc@label{\tl_use:N
    \l_csm_nomenclature_label_tl}%
  \edef\nomenc@width{\tl_use:N
    \l_csm_nomenclature_first_col_width_tl}%
  \edef\nomenc@position{\tl_use:N
    \l_csm_nomenclature_position_tl}%
  \def\@nomenclature@content{\BODY}
  % Write sidebar body to file
  \newwrite\file
  \immediate\openout\file=csm_\nomenc@label.tex
  \immediate\write\file{\noexpand\footnotesize}
  \immediate\write\file{\string\def\string\arraystretch{1.2}}
  \immediate\write\file{\string\newcolumntype{V}{%
      >{\string\hsize=\nomenc@width\string\linewidth}X}}
  \immediate\write\file{\string\begin{tabularx}{\string\columnwidth}{VX}}
  \immediate\write\file{  \string\input{#2}}
  \immediate\write\file{\string\end{tabularx}}
  \immediate\closeout\file
  % Push sidebar into queue
  \declaresidebar[%
  title={\nomenc@title},
  columns=1,
  label={\nomenc@label},
  position={\nomenc@position}]{csm_\nomenc@label.tex}
}

\makeatother
\ExplSyntaxOff

% ..:: Author biography ::..

\ifmakeprettycsm
\newenvironment{authorbio}[1][]{
  {\bfseries\itshape #1}~}{}
\else
\newenvironment{authorbio}[1][]{
  #1~}{}
\fi

% ..:: Bibliography ::..

\setlength{\biblabelsep}{1mm}
\setlength\bibitemsep{0.1\baselineskip}

% Remove hanging indent
% Source: https://tex.stackexchange.com/a/400666/90535
\defbibenvironment{bibliography}
{\list
  {\printtext[labelnumberwidth]{%
      \printfield{labelprefix}%
      \printfield{labelnumber}}}
  {\setlength{\labelwidth}{\labelnumberwidth}%
    \setlength{\leftmargin}{0pt}%{\labelwidth}%
    \setlength{\labelsep}{\biblabelsep}%
    \setlength{\itemsep}{\bibitemsep}%
    \setlength{\parsep}{\bibparsep}}%
  \renewcommand*{\makelabel}[1]{\hss\hspace{\dimexpr%
      \labelnumberwidth+\labelsep}##1}}
{\endlist}
{\item}

\newcommand{\csmprintmainbib}{%
  \begin{refcontext}[sorting=none]%
    \renewcommand*{\bibfont}{\footnotesize}%
    \DeclareFieldFormat{labelnumberwidth}{[##1]}%
    \printbibliography[notkeyword=sidebarbib, resetnumbers=true]%
  \end{refcontext}%
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> latex_common/elsevier_style.tex <==
% Font
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{microtype}
\let\acute\undefined
\let\grave\undefined
\let\ddot\undefined
\let\tilde\undefined
\let\bar\undefined
\let\breve\undefined
\let\check\undefined
\let\hat\undefined
\let\dot\undefined
\let\mathring\undefined
\let\wideparen\undefined
\usepackage{fouriernc} % Math and text font
\usepackage{charter} % Override text font

% Margins
\def\elsSideMargin{1.2cm}
\def\elsTopMargin{1.1cm}
\def\elsColSep{9.5mm}
\usepackage[left=\elsSideMargin,
right=\elsSideMargin,
top=\elsTopMargin,
bottom=\elsTopMargin,
columnsep=\elsColSep]{geometry}

% Line skip
\renewcommand{\baselinestretch}{0.9}

%%%%%%%%%%%%%%%%%%%%%%%
% Figures
%%%%%%%%%%%%%%%%%%%%%%%

\setlength{\mathindent}{0pt} % Left-justified math

%%%%%%%%%%%%%%%%%%%%%%%
% Figures
%%%%%%%%%%%%%%%%%%%%%%%

\captionsetup[figure]{labelfont={bf},font=footnotesize,name={Fig.},labelsep=period}

%%%%%%%%%%%%%%%%%%%%%%%
% Heading and footer
%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\listget}[3][]{\list@get[#1]{#2}{#3}}
\makeatother
\fancypagestyle{elsevierfancy}
{
  \fancyhf{}
  \renewcommand{\headrulewidth}{0pt}
  \fancyhead[L]{
    \footnotesize
    \thepage
  }
  \fancyhead[C]{
    \itshape
    \footnotesize
    \xdef\elscounter{1}
    \xdef\elsmaxauthor{3}
    \foreach \authorfullnameaffil in \elsauthorlist {%
      \listget[authorfullname]{\authorfullnameaffil}{2}%
      \StrLeft{\authorfullname}{1}[\authornamefirstchar]%
      \authornamefirstchar.~% % first name
      \elsgetlistelement{\authorfullname}{2}% % last name
      \pgfmathparse{\elscounter==\elsmaxauthor ? 1:0}%
      \ifthenelse{\pgfmathresult>0}{~et al.\breakforeach}{}%
      \pgfmathparse{\elscounter<min(\elsmaxauthor,\elsauthorcount)-1 ? 1:0}%
      \ifthenelse{\pgfmathresult>0}{,~}{}%
      \pgfmathparse{\elscounter==min(\elsmaxauthor,\elsauthorcount)-1 ? 1:0}%
      \ifthenelse{\pgfmathresult>0}{~and~}{}%
      \elsaddtocounter{\elscounter}%
    }
    / Annual Reviews in Control
  }
}
\headheight 28pt              %% put this outside
\headsep 10pt                 %% put this outside

\pagestyle{elsevierfancy}

%%%%%%%%%%%%%%%%%%%%%%%
% Section style
%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{indentfirst}
\setlength\parindent{5mm}

\titleformat{\section}{\normalfont\bfseries\normalsize}{}{0cm}{\thesection.~#1}
\titleformat{\subsection}{\normalfont\itshape\normalsize}{}{0cm}{\thesubsection.~#1}
\titleformat{\subsubsection}{\normalfont\itshape\normalsize}{}{0cm}{\thesubsubsection.~#1}
\titlespacing*{\section}{0cm}{8mm}{4mm}
\titlespacing*{\subsection}{0cm}{5mm}{5mm}
\titlespacing*{\subsubsection}{0cm}{5mm}{\lineskip}


%%%%%%%%%%%%%%%%%%%%%%%
% Document head
%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter
\newcommand{\elstitle}[1]{
  \def\@elstitle{#1}
}
\makeatother

\newcommand{\elsappendtolist}[2]{
  % #1: list
  % #2: element to add to end
  \ifthenelse{\equal{#1}{}}{\xdef#1{#2}}{\xdef#1{#1,#2}}
}

\makeatletter%
\newcommand{\elsgetlistelement}[2]{%
  % #1: list
  % #2: element index (1-indexing)
  \xdef\@@counter{1}%
  \foreach \element in #1 {%
    \pgfmathparse{\@@counter==#2 ? 1:0}%
    \ifthenelse{\pgfmathresult>0}{\element\breakforeach}{}%
    \elsaddtocounter{\@@counter}%
  }%
}
\makeatother%

\makeatletter%
\newcommand{\elsaddtocounter}[2][]{%
  \xdef\@increment{1}%
  \ifthenelse{\equal{#1}{}}{}{\xdef\@increment{#1}}%
  \tikzmath{#2=int(#2+\@increment);}%
  \xdef#2{#2}%
}
\makeatother%

\xdef\elsauthorlist{}
\xdef\elsaffiliationlist{}
\xdef\elsauthorcount{0}
\xdef\elsaffiliationcount{0}
\newcommand{\elsauthor}[2]{%
  \elsappendtolist{\elsauthorlist}{{#1,{#2}}}%
  \elsaddtocounter{\elsauthorcount}%
}
\newcommand{\elsaffiliation}[2]{%
  \elsappendtolist{\elsaffiliationlist}{{#1,{#2}}}%
  \elsaddtocounter{\elsaffiliationcount}%
}

\makeatletter
\define@key{@elspaperhead@keys}{received}{\def\@receive@date{#1}}
\define@key{@elspaperhead@keys}{revised}{\def\@revised@date{#1}}
\define@key{@elspaperhead@keys}{accepted}{\def\@accepted@date{#1}}
\define@key{@elspaperhead@keys}{available}{\def\@available@date{#1}}
\define@key{@elspaperhead@keys}{keywords}{\def\@keywords{#1}}
\NewEnviron{elspaperhead}[1][]{
  \setkeys{@elspaperhead@keys}{received=,#1}
  \setkeys{@elspaperhead@keys}{revised=,#1}
  \setkeys{@elspaperhead@keys}{accepted=,#1}
  \setkeys{@elspaperhead@keys}{available=,#1}
  \setkeys{@elspaperhead@keys}{keywords=,#1}
  
  \twocolumn[
  \begin{pykzpicture}

    \def\@vshift{4mm}
    \def\@logo@height{2cm}

    \tikzset{
      separator/.append style={
        line width=0.1mm
      },
      fatbar/.append style={
        line width=1mm,
        line cap=rect
      },
      review/.append style={
        scale=1.2,
        anchor=north west
      }
    }
    
    \@node{
      anchor=north west,
      yshift=-\@vshift
    } (elslogo) at (0,0)
    {\includegraphics[height=\@logo@height]{latex_common/media/elsevier_logo.pdf}};

    \@node{
      anchor=south east
    } (arcfp) at (\textwidth,-\@logo@height-\@vshift)
    {\includegraphics[height=\@logo@height+\@vshift]{latex_common/media/arc_fp.pdf}};

    \path let \p1=(arcfp.east), \p2=(arcfp.west) in \pgfextra{
      \tikzmath{\@H = \textwidth-(\x1-\x2)-\@vshift;}
      \dimensionalize{\@H}
      \@draw{separator} (0,0) -- ++(\@H,0) node(tmp){};
    };

    \path let \p1=(elslogo.south east), \p2=(tmp) in \pgfextra{
      \@draw{
        fill=black!20,
        draw=none} (\x1+\@vshift,\y1) rectangle (\x2,\y2-\@vshift);
      \@node{scale=1.7} at ({(\x1+\@vshift+\x2)/2},{(\y1+\y2-\@vshift)/2})
      {Annual Reviews in Control};
    };
    
    \@draw{fatbar} ($(elslogo.south west)+(0,-\@vshift)$) node(tmp){} -- ++(\textwidth,0);
    \@node{review} at ($(tmp)+(0,-5mm)$) {Review};
  \end{pykzpicture}
  
  \vspace{5mm}
  \thispagestyle{empty}
  {\LARGE\@elstitle}\medskip

  \xdef\@counter{1}
  \foreach \authorfullnameaffil in  \elsauthorlist {%
    \list@get[affiliation]{\authorfullnameaffil}{1}%
    \list@get[authorfullname]{\authorfullnameaffil}{2}%
    \large%
    {\color{black!50}\elsgetlistelement{\authorfullname}{1}}~% % first name
    \elsgetlistelement{\authorfullname}{2}$^{\text{
        \hyperlink{affil\affiliation}{\affiliation}
      }}$% % last name
    \pgfmathparse{\@counter<\elsauthorcount-1 ? 1:0}%
    \ifthenelse{\pgfmathresult>0}{,~}{}%
    \pgfmathparse{\@counter==\elsauthorcount-1 ? 1:0}%
    \ifthenelse{\pgfmathresult>0}{~and~}{}%
    \elsaddtocounter{\@counter}%
  }
  \vspace{3mm}

  \foreach \affiliation@details in \elsaffiliationlist {%
    \list@get[@letter]{\affiliation@details}{1}
    \list@get[@text]{\affiliation@details}{2}
    {\footnotesize\hypertarget{affil\@letter}{$^{\text{\@letter}}$}~\textit{\@text}}
  }
  \vspace{5mm}
  
  \def\@vsep@big{0.7cm}
  \def\@vsep@small{0.6*\@vsep@big}
  \def\@kw@width{0.25\textwidth}
  \def\@hsep{0.1\textwidth}

  \tikzmath{\@abstract@width=(\textwidth-\@kw@width-\@hsep)/0.9;}
  \dimensionalize{\@abstract@width}

  \newsavebox\Abstract
  \begin{lrbox}{\Abstract}
    \begin{minipage}{\@abstract@width}
      \BODY
    \end{minipage}
  \end{lrbox}

  \begin{pykzpicture}

    \tikzset{
      separator/.append style={
        line width=0.1mm
      },
      title/.append style={
        anchor=north west,
        scale=0.9
      },
      info text/.append style={
        scale=0.8,
        anchor=north west,
        yshift=-1mm
      },
      abstract/.append style={
        anchor=north west,
        align=left,
        yshift=-1mm,
        scale=0.9
      }
    }

    \@draw{separator} (0,0) -- ++(\textwidth,0);

    \@node{title} (info) at (0,-\@vsep@big) {A~R~T~I~C~L~E~~~~I~N~F~O};

    \@draw{separator}
    ($(info.south west)+(0,-\@vsep@small)$) --
    ++(\@kw@width,0);

    \@node{info text} (history) at ($(info.south west)+(0,-\@vsep@small)$)
    {\textit{Article history:}};
    \@node{info text} (received) at (history.south west) {Received
      \@receive@date};
    \@node{info text} (revised) at (received.south west) {Revised
      \@revised@date};
    \@node{info text} (accepted) at (revised.south west) {Accepted
      \@accepted@date};
    \@node{info text} (available) at (accepted.south west) {Available
      \@available@date};

    \@draw{separator} ($(available.south west)+(0,-\@vsep@small)$) --
    ++(\@kw@width,0);
    \@node{info text} (keywords_prev) at ($(available.south west)+(0,-\@vsep@small)$)
    {\textit{Keywords:}};

    \pykzmathinline{len([\@keywords])}
    \xdef\keywordlen{\out}

    \foreach \@i in {1,...,\keywordlen} {
      \pykzmathinline{([\@keywords])[\@i-1]}
      \@node{info text} (keywords_prev) at (keywords_prev.south west) {\out};
    }

    \@node{title} (abstract)
    at (\@kw@width+\@hsep,-\@vsep@big) {A~B~S~T~R~A~C~T};
    
    \@draw{separator} ($(info.south west)+(\@kw@width+\@hsep,-\@vsep@small)$) --
    ++(\textwidth-\@kw@width-\@hsep,0);

    \@node{abstract} (abstract) at ($(info.south west)+(\@kw@width+\@hsep,-\@vsep@small)$)
    {\usebox\Abstract};

    \@node{scale=0.9,anchor=north east,yshift=-1mm}
    (copyright)
    at (abstract.south east)
    {{\small\copyright}~ 2020 Elsevier Ltd. All rights reserved.};

    \@draw{separator} ($(copyright.north east)+(0,-\@vsep@big)$)
    -- ++(-\textwidth,0);
    
  \end{pykzpicture}

  \renewcommand*\l@section{\@dottedtocline{3}{0.5em}{2.3em}}
  \renewcommand\@dotsep{3}
  \renewcommand\tableofcontents{%
    \titleformat{\section}{\normalfont\bfseries\normalsize}{}{0cm}{Contents}
    \section*{\contentsname
      \@mkboth{%
        \MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
    \@starttoc{toc}%
  }
  % \renewcommand\cftchapafterpnum{\vskip10pt}
  \renewcommand\cftsecafterpnum{\vskip3pt}
  
  \tableofcontents

  \vspace{7mm}
  ]
}
\newcommand{\@node}[1]{\node[#1]}
\newcommand{\@draw}[1]{\draw[#1]}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%
% Bibliography
%%%%%%%%%%%%%%%%%%%%%%%

\def\elscitecolor{blue!60}
\setcitestyle{authoryear,semicolon}% ,open={((},close={))}}
\hypersetup{
  colorlinks,
  linkcolor={red},
  citecolor={\elscitecolor},
  urlcolor={blue}
}
\renewcommand*{\bibfont}{\footnotesize\color{\elscitecolor}}
\setlength{\bibsep}{1pt}

%%%%%%%%%%%%%%%%%%%%%%%
% Theorems
%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

\theoremstyle{definition}

\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{assumption}{Assumption}
\newtheorem{property}{Property}
\newtheorem{example}{Example}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/optimization.tex <==
\ExplSyntaxOn
\makeatletter

\def\objective@label{objective}

\tl_new:N \l_opti_task_tl
\tl_new:N \l_opti_label_tl
\tl_new:N \l_opti_vars_tl
\tl_new:N \l_opti_objective_tl
\tl_new:N \l_opti_result_tl

\define@key{optim@keys}{task}{\tl_set:Nn \l_opti_task_tl {#1}}
\define@key{optim@keys}{label}{\tl_set:Nn \l_opti_label_tl {#1}}
\define@key{optim@keys}{variables}{\tl_set:Nn \l_opti_vars_tl {#1}}
\define@key{optim@keys}{objective}{\tl_set:Nn \l_opti_objective_tl {#1}}
\define@key{optim@keys}{result}{\tl_set:Nn \l_opti_result_tl {#1}}

\newenvironment{optimization}[1][]{
  \setkeys{optim@keys}{task=\min,#1}
  \setkeys{optim@keys}{label=,#1}
  \setkeys{optim@keys}{variables=,#1}
  \setkeys{optim@keys}{objective=,#1}
  \subequations
  \label{problem:\tl_use:N \l_opti_label_tl}
  \align
  \optilabel{\objective@label}
  \ifthenelse{\equal{\tl_use:N \l_opti_result_tl}{}}{}{%
    \tl_use:N \l_opti_result_tl =}%
  \tl_use:N \l_opti_task_tl\c_math_subscript_token
  {\mathclap{\tl_use:N \l_opti_vars_tl}}\textnormal{\ }
  & \tl_use:N \l_opti_objective_tl \\
  \mrm[t]{s.t.}\textnormal{\ }
}{
  \endalign
  \endsubequations
}

\newenvironment{optimization*}[1][]{
  \setkeys{optim@keys}{task=\min,#1}
  \setkeys{optim@keys}{variables=,#1}
  \setkeys{optim@keys}{objective=,#1}
  \csname align*\endcsname
  \tl_use:N \l_opti_task_tl\c_math_subscript_token
  {\mathclap{\tl_use:N \l_opti_vars_tl}}\textnormal{\ }
  & \tl_use:N \l_opti_objective_tl \\
  \mrm[t]{s.t.}\textnormal{\ }
}{
  \csname endalign*\endcsname
}

\newcommand{\optilabel}[2][eq]{\label{#1:\tl_use:N \l_opti_label_tl _#2}}
\newcommand{\optieqref}[2]{\eqref{eq:#1_#2}}
\newcommand{\optiobjref}[1]{\eqref{eq:#1_\objective@label}}

\makeatother
\ExplSyntaxOff

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/review_commands.tex <==
\makeatletter

% ..:: Colors ::..

\definecolor{@review@yellow}{HTML}{f1d46a}
\definecolor{@review@blue}{HTML}{356397}
\definecolor{@review@green}{HTML}{5da9a1}
\definecolor{@review@red}{HTML}{db6245}

% ..:: Some TikZ elements ::..

\tikzset{
  every node/.style={
    inner sep=0,
    outer sep=0,
    minimum size=0
  },
  inline box/.style={
    rectangle,
    inner xsep=1mm,
    font=\normalfont\sffamily\small,
    minimum height=1em
  },
  delim line/.style={
    line width=1pt
  }
}

\def\@delim@line@height{0.8em}
\def\@delim@line@half@angle{60}
\tikzmath{
  \@delim@line@width=\@delim@line@height/2/tan(\@delim@line@half@angle);
}
\newcommand{\@delim@line}[2]{%
  \ifthenelse{\equal{#2}{open}}{\xdef\@x@sign{}}{\xdef\@x@sign{-}}%
  \protect\tikz[baseline=-0.5ex,line cap=round,line join=round]{%
    \protect\draw[delim line,#1]
    (\@x@sign\@delim@line@width pt,-\@delim@line@height/2) --
    (0,0) --
    (\@x@sign\@delim@line@width pt,\@delim@line@height/2);
  }%
}

% ..:: Diffs ::..

\def\@new@clr{@review@green}

\DeclareRobustCommand{\@new@box}{%
  \protect\tikz[baseline=-0.5ex]{%
    \protect\node[inline box,fill=\@new@clr,text=white] {new};
  }%
}

% Idea from: https://tex.stackexchange.com/a/23842/90535
\DeclareRobustCommand{\changed}[1]{%
  \texorpdfstring{%
    \@new@box~%
    \@delim@line{\@new@clr}{open}~%
    {\color{\@new@clr}#1}~%
    \@delim@line{\@new@clr}{close}}%
  {{\color{\@new@clr}#1}}}

% For \leavvmode: https://tex.stackexchange.com/a/207228/90535
\newenvironment{changedblock}{%
  \@new@box~%
  \@delim@line{\@new@clr}{open}~%
  \leavevmode\color{\@new@clr}\ignorespaces%
}{\@delim@line{\@new@clr}{close}}

\def\beginchange{\begin{changedblock}}
\def\endchange{\end{changedblock}}

\makeatother

% ..:: Comments ::..

% >> Question <<

\makeatletter

\def\@question@clr{@review@green}

\DeclareRobustCommand{\@question@box}{%
  \protect\tikz[baseline=-0.5ex]{%
    \protect\node[inline box,fill=\@question@clr,text=white] {question};
  }%
}

\DeclareRobustCommand{\question}[2]{%
  \def\@text{#1}%
  \def\@question{#2}%
  \texorpdfstring{%
    \@question@box~%
    \@delim@line{\@question@clr}{open}~%
    {\color{\@question@clr}\@text}~%
    \@delim@line{\@question@clr}{close}%
    {\sffamily\footnotesize\color{\@question@clr}\textbf{:}~\@question}%
  }%
  {{\color{\@question@clr}\@text}}}

\makeatother

% >> Fix <<

\makeatletter

\def\@fixme@clr{@review@red}

\DeclareRobustCommand{\@fixme@box}{%
  \protect\tikz[baseline=-0.5ex]{%
    \protect\node[inline box,fill=\@fixme@clr,text=white] {fixme};
  }%
}

\DeclareRobustCommand{\fixme}[2]{%
  \def\@text{#1}%
  \def\@comment{#2}%
  \texorpdfstring{%
    \@fixme@box~%
    \@delim@line{\@fixme@clr}{open}~%
    {\color{\@fixme@clr}\@text}~%
    \@delim@line{\@fixme@clr}{close}%
    {\sffamily\footnotesize\color{\@fixme@clr}\textbf{:}~\@comment}%
  }%
  {{\color{\@fixme@clr}\@text}}}

\makeatother

% >> Todo <<

\makeatletter

\def\@todo@clr{@review@yellow}
\def\@todo@text@clr{@review@blue}

\DeclareRobustCommand{\@todo@box}{%
  \protect\tikz[baseline=-0.5ex]{%
    \protect\node[inline box,fill=\@todo@clr,text=black] {todo};
  }%
}

\DeclareRobustCommand{\todo}[2][]{%
  \def\@text{#1}%
  \def\@comment{#2}%
  \texorpdfstring{%
    \@todo@box~%
    \ifthenelse{\equal{\@text}{}}{}{%
      \@delim@line{\@todo@clr}{open}~%
      {\color{\@todo@text@clr}\@text}~%
      \@delim@line{\@todo@clr}{close}%
    }%
    \ifthenelse{\equal{\@comment}{}}{}{%
      {\sffamily\footnotesize\color{\@todo@text@clr}\textbf{:}~\@comment}}%
  }%
  {{\color{\@todo@text@clr}\@text}}}

\makeatother

% >> Bookmark <<

\makeatletter

\def\@bookmark@clr{@review@blue}

\DeclareRobustCommand{\@bookmark@box}{%
  \protect\tikz[baseline=-0.5ex]{%
    \protect\node[inline box,fill=\@bookmark@clr,text=white] {bookmark};
  }%
}

\DeclareRobustCommand{\bookmark}[2][]{%
  \def\@text{#1}%
  \def\@comment{#2}%
  \texorpdfstring{%
    \@bookmark@box~%
    \ifthenelse{\equal{\@text}{}}{}{%
      \@delim@line{\@bookmark@clr}{open}~%
      {\@text}~%
      \@delim@line{\@bookmark@clr}{close}%
    }%
    \ifthenelse{\equal{\@comment}{}}{}{%
      {\sffamily\footnotesize\textbf{:}~\@comment}}%
  }{\@text}}

\makeatother

% ..:: Old ::..

\def\removeColor{red}
\def\changeColor{orange}
\def\commentColor{green}

\newcommand{\reviewAddToList}[2]{%
  % #1: list variable
  % #2: element
  \ifthenelse{\equal{#1}{}}{\xdef#1{#2}}{\xdef#1{#1,#2}}%
}

\makeatletter
\define@key{removeKeys}{style}{\def\style{#1}}%
\makeatother
\newcommand{\remove}[2][]{%
  \setkeys{removeKeys}{style=-,#1}%
  {%
    \color{\removeColor}%
    \ifthenelse{\equal{\style}{/}}{%
      \cancel{#2}%
    }{%
      \sout{#2}%
    }%
  }%
}

\newcommand{\addin}[1]{%
  {%
    \color{\commentColor}%
    {#1}%
  }%
}

\newcommand{\change}[2]{%
  {%
    \color{\removeColor}%
    \remove{#1}~%
  }{%
    \color{\changeColor}%
    #2%
  }%
}

\xdef\reviewCommentCounter{0}
\xdef\reviewCommentList{}
\makeatletter
\define@key{commentKeys}{txt}{\def\txt{#1}}%
\define@key{commentKeys}{inline}{\def\inline{#1}}%
\makeatother
\newcommand{\commentBoxName}[1]{CommentBox#1}
\renewcommand{\comment}[2][]{%
  \setkeys{commentKeys}{txt=,#1}%
  \setkeys{commentKeys}{inline=f,#1}%
  \def\InsertText{\color{black}\txt}
  \tikzmath{\reviewCommentCounter=int(\reviewCommentCounter+1);}%
  \xdef\reviewCommentCounter{\reviewCommentCounter}%
  {%
    \color{\commentColor}%
    [#2]$^{\textnormal{\hyperlink{commentRef\reviewCommentCounter}{\reviewCommentCounter}}}$%
  }%
  \ifthenelse{\equal{\inline}{f}}{%
    \edef\BoxName{\csname \commentBoxName{\reviewCommentCounter}\endcsname}%
    \expandafter\newsavebox\BoxName%
    \begin{lrbox}{\BoxName}%
      \begin{minipage}{\textwidth}%
        \normalsize\InsertText%
      \end{minipage}%
    \end{lrbox}%
    \global%
    \expandafter\setbox\BoxName%
    \expandafter\box\BoxName%
    \reviewAddToList{\reviewCommentList}%
    {\reviewCommentCounter/\commentBoxName{\reviewCommentCounter}}%
  }{%
    \pgfmark{commentPos\reviewCommentCounter}%
    \begin{tikzpicture}[
      overlay,
      remember picture
      ]%
      \tiklzcommonsettings
      \tikzmath{
        \leftpad=3mm;
      }
      \tikzset{
        sidebar comment/.append style={
          \commentColor,
          anchor=north west,
          align=left,
          text width=2cm
        }
      }
      \path let
      \p1=(current page.west),
      \p2=(pic cs:commentPos\reviewCommentCounter)
      in \pgfextra{
        \node[sidebar comment] at (\x1+\leftpad pt,\y2+0.7em)
        {\footnotesize$^{\hypertarget{commentRef\reviewCommentCounter}{\reviewCommentCounter}}$
          \InsertText};
      };
    \end{tikzpicture}%
  }%
}
\newcommand{\printCommentList}{
  \section*{\color{\commentColor}Comments}
  \foreach \commentNumber/\commentText in \reviewCommentList {

    \hypertarget{commentRef\commentNumber}{\textbf{Comment \commentNumber:}}
    \medskip

    \edef\GetBox{\expandafter\usebox\csname \commentText\endcsname}
    \GetBox
    \medskip
  }
}

%%%%%%%%%%%%%%%%%%%%%%%% OLD

\definecolor{darkolivegreen}{rgb}{0.33, 0.6, 0.18}
% \definecolor{green}{rgb}{0, 0.5, 0}
\definecolor{orange}{rgb}{1, 0.4, 0}
\definecolor{darkgray}{rgb}{0.2, 0.2, 0.2}

\newcommand{\seecode}{\textit{For code, see Appendix~\ref{sec:code}}.}
\newcommand{\postmeeting}[2][show]{%
  \ifthenelse{\equal{#1}{show}}{%
    {\color{orange} #2}%
  }{}%
}
\newcommand{\idea}[2][show]{%
  \ifthenelse{\equal{#1}{show}}{%
    {\color{orange} #2}%
  }{}%
}
\newcommand{\mycomment}[2][show]{%
  \ifthenelse{\equal{#1}{show}}{%
    {\color{red} (C: #2)}%
  }{}%
}

\newcommand\dangersign[1][2ex]{%
  \renewcommand\stacktype{L}%
  \scaleto{\stackon[1.3pt]{\color{red}$\triangle$}{\tiny !}}{#1}%
}
\newcommand{\marginwarning}[1]{\marginnote{\footnotesize\dangersign{\color{red}#1}}}
\newcommand{\margindate}[1]{\marginnote{\footnotesize\color{red}\texttt{#1}}}
\newcommand{\easy}{{\color{olive}[easy]}\xspace}
\newcommand{\moderate}{{\color{orange}[moderate]}\xspace}
\newcommand{\hard}{{\color{red}[hard]}\xspace}
\newcommand{\stoppedhere}{{\color{red}\bfseries STOPPED~HERE}\xspace}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> latex_common/review_response.tex <==
\makeatletter

% ..:: Colors ::..

\definecolor{@response@darkblue}{HTML}{26415d}
\definecolor{@response@blue}{HTML}{356397}
\definecolor{@response@green}{HTML}{5da9a1}
\definecolor{@response@yellow}{HTML}{f1d46a}
\definecolor{@response@red}{HTML}{db6245}
\definecolor{@response@black}{HTML}{000000}
\definecolor{@response@grey}{HTML}{acacac}

% ..:: Page geometry ::..

\def\side@margin{3cm}
\def\top@margin{2cm}
\usepackage[left=\side@margin,
right=\side@margin,
top=\top@margin,
bottom=\top@margin]{geometry}

% ..:: Some inline TikZ options ::..

\tikzset{
  response box/.style={
    fill=@response@blue,
    text=white,
    font=\sffamily,
    inner sep=1mm
  },
  section box/.style={
    fill=@response@red,
    text=white,
    font=\sffamily,
    inner sep=2mm
  },
  title box/.style={
    fill=@response@green,
    text=white,
    font=\sffamily\bfseries,
    inner sep=2mm,
    scale=1.2,
    minimum height=8mm
  },
  date box/.style={
    title box,
    fill=@response@yellow,
    text=black,
    font=\sffamily\footnotesize
  },
  every node/.append style={
    inner sep=0,
    outer sep=0,
    minimum size=0
  }
}

% ..:: Section style ::..

\newcommand{\@section@title}[2]{%
  \tikz[baseline=-0.5ex]{%
    \node[section box] {#2};
  }%
}

\usepackage{helvet}
\titleformat{\section}{%
  \normalfont\fontsize{10}{12}%
  \sffamily\bfseries}{}{0cm}{%
  \@section@title{@response@red}{\MakeUppercase{#1}}}
\titlespacing*{\section}{0cm}{10mm}{0mm}

\titleformat{\subsection}{%
  \normalfont\fontsize{10}{12}%
  \sffamily\bfseries\slshape}{}{0cm}{#1}
\titlespacing*{\subsection}{0cm}{4mm}{0mm}

\titleformat{\subsubsection}{%
  \normalfont\fontsize{10}{12}%
  \sffamily}{}{0cm}{#1}
\titlespacing*{\subsubsection}{0cm}{4mm}{0mm}

% ..:: Title text ::..

\newcommand{\reviewheader}{%
  \tikz[baseline=-0.5ex]{%
    \node[title box] {Responses to Editor and Reviewer Comments};
  }%
  \hfill%
  \tikz[baseline=-0.5ex]{%
    \node[date box] {\today};
  }%
}

\newtcolorbox{subtitle@box}{
  % Drawing engine
  enhanced jigsaw,
  breakable,
  % Sizes
  width=\linewidth,
  boxrule=0pt,
  titlerule=0pt,
  arc=0mm,
  left=2mm,
  right=2mm,
  bottom=1mm,
  top=1mm,
  boxsep=1mm,
  % Fonts
  fontupper=\sffamily,
  % Colors
  colback=black!10,
  coltext=black
}

\newcommand{\papername}[1]{%
  \begin{subtitle@box}
    #1
  \end{subtitle@box}%
}

\newcommand{\authorlist}[1]{%
  {\small\itshape #1}%
}

\newenvironment{reviewabstract}{%
}{}

% ..:: Reviewer text box ::..

\newtcolorbox{review@text@box}{
  % Drawing engine
  enhanced jigsaw,
  breakable,
  % Sizes
  width=\linewidth,
  boxrule=0pt,
  titlerule=0pt,
  arc=0mm,
  left=3mm,
  right=3mm,
  bottom=3mm,
  top=3mm,
  boxsep=1mm,
  % Colors
  colback=black!10
}

\newenvironment{reviewtext}{%
  \begin{review@text@box}%
  }{%
  \end{review@text@box}%
}

% ..:: Response text ::..

\newcommand{\@author@response}{%
  \tikz[baseline=-0.5ex]{%
    \node[response box] {Response};
  }}

\newenvironment{response}{%
  \@author@response~%
}{%
}

% ..:: Text quotes ::..

\newtcolorbox{quote@text@box}{
  % Drawing engine
  enhanced jigsaw,
  breakable,
  % Sizes
  width=\linewidth,
  boxrule=0pt,
  leftrule=2pt,
  titlerule=0pt,
  arc=0mm,
  left=3mm,
  right=1mm,
  bottom=1mm,
  top=1mm,
  boxsep=1mm,
  % Colors
  opacityback=0,
  colframe=@response@green
}

\newenvironment{paperquote}{%
  \begin{quote@text@box}%
    \color{black!60}
  }{%
  \end{quote@text@box}%
}

% ..:: Bibliography ::..

\def\elscitecolor{blue!60}
\setcitestyle{authoryear,semicolon}
\hypersetup{
  colorlinks,
  linkcolor={red},
  citecolor={\elscitecolor},
  urlcolor={blue}
}
\renewcommand*{\bibfont}{\footnotesize\color{\elscitecolor}}
\setlength{\bibsep}{1pt}

\makeatother

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

